Multi-Agent Generative Adversarial Imitation Learning

Imitation learning algorithms can be used to learn a policy from expert demonstrations without access to a reward signal. However, most existing approaches are not applicable in multi-agent settings due to the existence of multiple (Nash) equilibria and non-stationary environments. We propose a new framework for multi-agent imitation learning for general Markov games, where we build upon a generalized notion of inverse reinforcement learning. We further introduce a practical multi-agent actor-critic algorithm with good empirical performance. Our method can be used to imitate complex behaviors in high-dimensional environments with multiple cooperative or competing agents.

==> 6_discussion.tex <==
\section{Discussion}
We propose a model-free imitation learning algorithm for multi-agent settings that leverages recent advances in adversarial training; the algorithm is agnostic to the competitive/noncompetitive structure of the environment, but allows for incorporating a prior when it is available. Experimental results demonstrate that it is able to imitate complex behaviors in high-dimensional environments with both cooperative and adversarial interactions.
%While the proposed approach allows us to recover the expert policy, there are two main limitations. On the one hand, we are not considering the entire space of $\mb{MAIRL}(\pi_E)$ or even verifying that $\min f_r(\pi_E, V)$ is zero for all proposed reward functions. On the other hand, the problem with MARL being non-injective persists, and training an entirely new policy over the recovered rewards could still lead to policies that do not behave like experts; it might be possible to use an ensemble of reward functions to prevent this.
%%However, under the current assumptions, this seems to be a necessary sacrifice for computational efficiency. 
An interesting research direction is to explore new techniques for gathering expert demonstration; for example, when the expert is allowed to aid the agents by participating in part of the agent's learning process~\citep{hadfield2016cooperative}. 

==> arXiv Submission/1_introduction.tex <==
\section{Introduction}
Reinforcement learning (RL) methods are becoming increasingly successful at optimizing reward signals in complex, high dimensional environments~\citep{espeholt2018impala}. 
A key limitation of RL, however, is the difficulty of designing suitable reward functions for complex and not well-specified tasks~\citep{hadfield2017inverse,amodei2016concrete}. If the reward function does not cover all important aspects of the task, the agent could easily learn undesirable behaviors~\citep{amodei2016faulty}.
This problem is further exacerbated in multi-agent scenarios, such as multiplayer games~\citep{peng2017multiagent}, multi-robot control~\citep{matignon2012coordinated} and social interactions~\citep{leibo2017multi}; in these cases, agents do not even necessarily share the same reward function, especially in competitive settings where the agents might have conflicting rewards. 
% \s{mention competition?} 

Imitation learning methods address these problems via expert demonstrations~\citep{ziebart2008maximum,englert2015inverse,finn2016guided,stadie2017third}; the agent 
directly learns desirable behaviors by imitating an expert. Notably, inverse reinforcement learning~(IRL) frameworks assume that the expert is (approximately) optimizing an underlying reward function, and attempt to recover a reward function that rationalizes the demonstrations; an agent policy is subsequently learned through RL~\citep{ng2000algorithms,abbeel2004apprenticeship}. % The learned reward function can also be utilized to evaluate performance of other agents. 
Unfortunately, this paradigm is not suitable for general multi-agent settings 
due to environment being non-stationary to individual agents~\citep{lowe2017multi} and the existence of multiple equilibrium solutions~\citep{hu1998multiagent}. The optimal policy of one agent could depend on the policies of other agents, and vice versa, so there could exist multiple solutions in which each agents' policy is the optimal response to others. 
% \s{add an extra sentence here, explaining. why are there mulple solutions? why is non-stationarity a problem?} \s{maybe move this sentence after introducing what multi-agent imitation is}


In this paper, we propose a new framework for multi-agent imitation learning -- provided with demonstrations of a set of experts interacting with each other within the same environment, we aim to learn multiple parametrized policies that imitate the behavior of each expert respectively. 
% \s{define the problem: we are given demonstrations of experts interacting with each other. want to learn policies that imitate the behavior}
Using the framework of Markov games,
we integrate 
% Our method is based on combining 
multi-agent RL with a suitable extension of multi-agent inverse RL. The resulting procedure strictly generalizes Generative Adversarial Imitation Learning (GAIL,~\citep{ho2016generative}) in the single agent case. 
Imitation learning corresponds to a two-player game between a generator and a discriminator. The generator controls the policies of all the agents in a distributed way, and the discriminator contains a classifier for each agent that is trained to distinguish that agent's behavior from that of the corresponding expert. Upon training, the behaviors produced by the policies are indistinguishable from the training data through the discriminator.
% \s{upon training, behaviors produced by the generator are indistinguishable from the training data}
We can incorporate prior knowledge into the discriminators,
including the presence of cooperative or competitive agents.
In addition, we propose a novel multi-agent natural policy gradient algorithm that addresses the issue of high variance gradient estimates commonly observed in reinforcement learning~\citep{lowe2017multi,foerster2016learning}.
Empirical results demonstrate that our method can imitate complex behaviors in high-dimensional environments, such as particle environments and cooperative robotic control tasks, with multiple cooperative or competitive agents; the imitated behaviors are close to the expert behaviors with respect to ``true'' reward functions which the agents do not have access to during training. 
%\s{give a preview here. this sentence is not very informative. which environments? how well does it work?}

% \s{fix bibliography}

==> arXiv Submission/2_background.tex <==
\section{Preliminaries}
\subsection{Markov games}
We consider an extension of Markov decision processes (MDPs) called Markov 
%(stochastic) 
games~\citep{littman1994markov}. A Markov game~(MG) for $N$ agents is defined via a set of states $\mc{S}$, $N$ sets of actions $\{\mc{A}_i\}_{i=1}^{N}$. The function $T: \mc{S} \times \mc{A}_1 \times \cdots \times \mc{A}_N \to \mc{P}(\mc{S})$ describes the (stochastic) transition process between states, where $\mc{P}(\mc{S})$ denotes the set of probability distributions over the set $\mc{S}$. Given that we are in state $s_t$ at time $t$, the agents take actions $(a_1, \ldots, a_N)$ and the state transitions to $s_{t+1}$ with probability $T(s_{t+1} | s_t, a_1, \ldots, a_N)$.

Each agent $i$ obtains a (bounded) reward given by a function $r_i: \mc{S} \times \mc{A}_1 \times \cdots \times \mc{A}_N \to \bb{R}$.
% \s{given that we are in state $s$, agents take actions ..., the state transitions to .. with prob T()}
%, which could be parametrized by $\theta_i$ \s{parameters?}\js{yeah; not sure ``could'' is strong enough - I mean you can parametrize it or not but if you do then we call it $\theta_i$}. 
Each agent $i$ aims to maximize its own total expected return $R_i = \sum_{t=0}^{\infty} \gamma^t r_{i,t}$, where $\gamma$ is the discount factor and $T$ is the time horizon, by selecting actions through a (stationary and Markovian) %\s{stationary, markovian}
% \hr{$T$ denotes time horizon in this paragraph and the state transition function in the first paragraph?}
stochastic policy $\pi_i: \mc{S} \times \mc{A}_i \to [0, 1]$. The initial states are determined by a distribution $\eta: \mc{S} \to [0, 1]$.
%\s{joint policy not defined}

The joint policy is defined as $\piv(a \vert s) = \prod_{i=1}^{N} \pi_i(a_i \vert s)$, where we use bold variables without subscript $i$ to denote the concatenation of all variables for all agents
% \s{can we use bold for joint vectors throught the paper?}\js{okay, but probably just for pi, r, a and only when we explicitly deal with multi-agents}
%, and for variables in MDPs 
(e.g. $\piv$ denotes the joint policy $\prod_{i=1}^{N} \pi_i$ in a multi-agent setting, $\rv$ denotes all rewards, $\av$ denotes actions of all agents).
%or the policy for single-agent MDPs)

We use expectation with respect to a policy $\pi$ to denote an expectation with respect to the trajectories it generates. For example, $$\bb{E}_\pi\left[r(s, a)\right]\triangleq\bb{E}_{s_t, a_t \sim \pi}\left[\sum_{t=0}^\infty\gamma^tr(s_t, a_t)\right]$$
denotes the following sample process for the right hand side: $s_0 \sim \eta$, $a_{t} \sim \pi(a_t | s_t)$, $s_{t+1} \sim T(s_{t+1} | a_t, s_t)$, yet if we do not take expectation over the state $s$, then
$$\bb{E}_\pi\left[r(s, a) + \sum_{s' \in \mc{S}} T(s'|s, a) v(s')\right] \triangleq \bb{E}_{a \sim \piv(\cdot|s)}\left[r(s, a) + \sum_{s' \in \mc{S}} T(s'|s, a) v(s')\right]$$ assumes the policy samples only the next-step action $a$.
% \s{maybe add a description in words of what this process is. it's important to make sure folks get the notation right..}
%\s{description incomplete? looks single agent}\js{without subscript this means ``joint''?}.  
% \s{is this thing a vector?}\js{lets just treat vectors that has the agents dimension N?}
% \hr{Should $s$ and $a$ be bold in both equations, meaning the state and action for all agents?} agents share state i think, and here I guess it is not super necessary to use MA notations.

We use subscript $-i$ to denote \emph{all agents except for $i$}. For example, $(a_i, a_{-i})$ represents $(a_1, \ldots, a_N)$, the actions of all $N$ agents.
% \s{get rid of observations?}
% \s{if time, can be made cleaer using bold for joint vars}
% \subsection{Policy Gradient Methods}
% Policy gradient methods~\citep{williams1992simple,sutton2000policy} updates the parameters $\theta$ in order to maximize the expected return $R(\theta) = \bb{E}_{\pi}[r(s, a)]$:
% $$
% \nabla_\theta R(\theta) = \bb{E}_\pi \big[\sum_{t=0}^{T} \nabla_\theta \pi_\theta(\av_t \vert o_t) A(t) \big]
% $$
% where $A(t)$ is often chosen to be the advantage function $A^\piv(s_t, \av_t)$. For example, the advantage actor critic methods~\citep{mnih2016asynchronous} defines the advantage function as $k$-step returns with function approximation,
% $$
% A^\piv(o_t, \av_t) = \sum_{i=0}^{k-1} \big(\gamma^i r(s_{t+i}, a_{t+i}) + \gamma^k V_\phi^\piv(o_{t+k}) \big) - V_\phi^\piv(o_t)
% $$
% where $V_\phi^\pi$ is the value network that provides an estimate of the $\gamma$-discounted rewards from the policy $\pi$. 

% \subsection{Multi-Agent Actor Critic}
% \s{how is the davantage defined in multiagent setting? i thought you need some special definition (as in hu paper)}
% In Markov games, the agent's reward also depends on other agent's policies. This would further increase the variance in policy gradient estimates that are already noisy. In particular, \citet{lowe2017multi} show an example where the probability of moving in the right direction decreases exponentially with the number of agents. To deal with this issue, they introduce a centralized critic that receives additional information from other agents during training. For each agent, $A(t)$ is the estimated Q-value for $\pi_i$ that takes $(o_1, \ldots, o_N, a_1, \ldots, a_N)$ as input. This allows agents to learn its Q-value separately over arbitrary reward structures in the Markov game. Similar ideas have been discussed in ~\citep{foerster2017counterfactual}.
\subsection{Reinforcement learning and Nash equilibrium}
In reinforcement learning (RL), the goal of each agent is to maximize total expected return $\bb{E}_{\pi}[r(s, a)]$ given access to the reward signal $r$. In single agent RL, an optimal Markovian policy exists but the optimal policy might not be unique (e.g., all policies are optimal for an identically zero reward; see \citet{sutton1998reinforcement}, Chapter 3.8).
An entropy regularizer can be introduced to resolve this ambiguity. The optimal policy is found via the following RL procedure:
\begin{equation}
\mb{RL}(r) = \argmax_{\pi \in \Pi} H(\pi) + \bb{E}_\pi[r(s, a)],
\end{equation}
where $H(\pi)$ is the $\gamma$-discounted causal entropy~\citep{bloem2014infinite} of policy $\pi \in \Pi$.
\begin{definition}[$\gamma$-discounted Causal Entropy]
The $\gamma$-discounted causal entropy for a policy $\pi$ is defined as follows:
$$H(\pi) \triangleq \bb{E}_{\pi}[-\log \pi(a \vert s)] = \bb{E}_{s_t, a_t \sim \pi}\left[-\sum_{t=0}^\infty\gamma^t\log \pi(a_t| s_t)\right]$$
\end{definition}

% \s{missing a log?}
% \s{add a definition, explain what this is, why is resolves ambiguity}
If we scale the reward function by any positive value, the addition of $H(\pi)$ resolves ambiguity by selecting the policy among the set of optimal policies that have the highest causal entropy\footnote{For the remainder of the paper, we may use the term ``entropy'' to denote the $\gamma$-discounted causal entropy for policies.} -- the policy with both the highest reward and the highest entropy is unique because the entropy function is concave with respect to $\pi$ and the set of optimal policies is convex.  
%, and $\Pi$ is the set of all possible policies. 
%$H(\pi)$ encourages learning policies that have higher entropy, and resolves the ambiguity when multiple policies achieve the same optimal expected reward.

In Markov games, however, the optimal policy of an agent depends on other agents' policies. % that change during training. %~\citet{hu1998multiagent} 
One approach is to 
%replace the concept of optimality %(which is central to MDPs) with 
use 
an equilibrium solution concept, such as Nash equilibrium~\citep{hu1998multiagent}.
Informally, a set of policies $\{\pi_i\}_{i=1}^{N}$ is a Nash equilibrium if no agent can achieve higher reward by unilaterally changing its policy, i.e. $\forall i \in [1, N], \forall \hat{\pi}_i \neq \pi_i, \bb{E}_{\pi_i, \pi_{-i}}[r_i] \geq \bb{E}_{\hat{\pi}_i, \pi_{-i}}[r_i]$.
% This defines a stationary point for multiple agents within a Markov game, similar to the role of optimal policies in MDPs -- once all agents reach this point, they will not change their policies by learning alone.
The process of finding a Nash equilibrium can be defined as a constrained optimization problem~(\citet{filar2012competitive}, Theorem 3.7.2):
% \s{cite which theorem}
% We slightly abuse notations in RL, and let $Q_i(s, \pi)$ be the Q-function for agent $i$ by selecting the stochastic policy $\pi_i$ when other agents select $\pi_{-i}$, and $V_i(s, \pi_{-i})$ be the value function of $i$ (by taking expectation over $\pi_i(a \vert o)$). 
% The objective is then:
\begin{gather}
\min_{\pi \in \Pi, \vv \in \bb{R}^{\mc{S} \times N}} f_r(\pi, \vv) = \sum_{i=1}^{N} \left(\sum_{s \in \mc{S}} v_i(s) - \bb{E}_{a_i \sim \pi_i(\cdot | s)} q_i(s, a_i) \right)  \label{eq:marl} \\
v_i(s) \geq q_i(s, a_i) \triangleq \bb{E}_{\pi_{-i}}\left[r_i(s, \av) + \gamma \sum_{s' \in \mc{S}} T(s'|s, \av) v_i(s')\right] \quad \forall i \in [N], s \in \mc{S}, a_i \in \mc{A}_i \label{eq:q} \\
\av \triangleq (a_i, a_{-i}) \triangleq (a_1, \ldots, a_N) \qquad \vv \triangleq [v_1; \ldots; v_N] \nonumber
\end{gather}
% \s{at least once in the paper, i think we should spell out the longer equation with $a=(a_i,a_{-i})$. provide both the short one (what you have) and the long one}
% \s{improve fromatting. use slash left for parenthesis}
% \s{people might not realize that $v_i(s)$ is a component of $v$}
% \s{using boldface could help}
%\s{add sets after quantifiers, eg $\forall i \in [N]$}
%where $v_i: \mc{S} \to \bb{R}$ (not necessarily value function) and
where the joint action $\av$ includes actions $a_{-i}$ sampled from $\pi_{-i}$ and $a_i$. Intuitively, $\vv$ could represent some estimated value function for each state and $\qv$ represents the $Q$-function that corresponds to $\vv$.
% \s{$a$ is undefined. should clarify how it is built (expectation and ai)} \js{done}
% is the expectation of $v(s')$ for next state $s'$ when the $i$-th agent takes action $i$ and other agents use policy $\pi_{-i}$. 
% \s{add intuitive explanation for what $v$, q are}
The constraints enforce the Nash equilibrium condition -- when the constraints are satisfied, $(v_i(s) - q_i(s, a_i))$ is non-negative for every $i \in [N]$. Hence $f_r(\piv, \vv)$ is always non-negative for a feasible $(\piv, \vv)$. Moreover, this objective has a global minimum of zero if a Nash equilibrium exists, and $\pi$ forms a Nash equilibrium if and only if $f_r(\piv, \vv)$ reaches zero while being a feasible solution~(\citet{prasad2015study}, Theorem 2.4).  %Intuitively, this problem requires each agent to find the best response to other agents' policies.
% \s{qi def is a bit sloppy because $a$ is undefined. i'm assuming $a=(a_i,a_{-i})$?}\js{a = all actions by definition in MG section?}
%\s{this def doesn't type check. V depends on a policy in (1)? only the minimum V depends on policy?}
%\s{what is the domain of $V$ in the min?}
%\s{add a paragraph explaining what this does}
% \s{wrap this into a definition of MARL. its a key concept and we want reader to pay attention}
% \dl{formal definition of $r$? set of all $r_i$?}\js{see MG section maybe I should emph that more?}\dl{I saw the one for $r_i$ not $r$} 

% This objective has a global minimum of zero. $\pi$ form a Nash equilibrium if and only if $f_r(\pi, V)$ reaches zero while being a feasible solution~\citep{prasad2015study}. Intuitively, this problem requires each agent to find the best response to other agents' policies.

% In game theory, strategies that constitute a Nash equilibrium can be time-dependent; an agent could select its policy according to the history of interactions with other agents. The strategies defined through the policies $\piv(a \vert o)$ in Markov games belong to a smaller category called stationary strategies, i.e. the policy only depends on the current state. Equilibria based on such strategies are called stationary Markov perfect equilibria; we only consider learning such equilibria for the remainder of the paper. Moreover, we assume that a stationary Markov perfect equilibrium exists for any Markov games that we encounter; the reader can refer to~\citep{he2017stationary} for a discussion of the existence of such equilibria in general-sum Markov games. \js{appendix}

% \s{brief section on $RL$ and $MARL$ operators}
% \s{given access to reward signal, objective is to maximize reward}

% \s{single agent. existence of optimal markovian policy. not necessarily unique}

% \s{multiagent. equilibria. non uniqueness. copy over the constrained objective. define marl} \js{should we define marl here? }
% Solving the problem in Eq.~\ref{eq:marl} is complicated by the fact that these constraints are non-convex. In general Markov games, gradient methods can converge to a local minimum but not the global minimum~\citep{prasad2015study} and hence convergence to a Nash equilibrium is not guaranteed. While one could use concepts such as $\epsilon$-Nash equilibrium for local optima~\citep{filar2012competitive}, we assume RL methods can converge to Nash equilibria for ease of exposition in this paper and let $\mb{MARL}(r)$ be the set of policies that are globally optimal to the objective in Eq.~\ref{eq:marl}:


\subsection{Inverse reinforcement learning}
%\s{define expert policy}
% \s{assume we don't have access to the reward (sorry, typo before)}
Suppose we do not have access to the reward signal $r$, but have demonstrations $\mc{D}$ provided by an expert ($N$ expert agents in Markov games). Imitation learning aims to learn policies that behave similarly to these demonstrations. % In a single-agent case, the demonstrations form a dataset of state-action pairs $\mc{D} = \{(s_j, a_j)\}_{j=1}^{M}$, where $a_j$ is obtained navigating the environment using an (unknown) expert policy $\pi_E$. 
In Markov games, we assume all experts/players operate in the same environment, and the demonstrations $\mc{D} = \{(s_j, a_j)\}_{j=1}^{M}$ are collected by sampling $s_0 \sim \eta(s), \av_t = \pi_E(\av_t \vert s_t), s_{t+1} \sim T(s_{t+1} \vert s_t, \av_t)$; we assume knowledge of $N$, $\gamma$, $\mc{S}$, $\mc{A}$, as well as access to $T$ and $\eta$ as black boxes. %subsequently \s{define formally. this is important, it's the key input to the algorithm}. 
% \s{again, use bold. remind reader that these are joints over all players}
% We assume kn;
We further assume that once we obtain $\mc{D}$, we cannot ask for additional expert interactions with the environment (unlike in DAgger~\citep{ross2011reduction} or CIRL~\citep{hadfield2016cooperative}).
% \s{say explicitly what is known and what is unknown, accessible through samples, for the markov game. we know $N$, $\gamma$(?), $S$, action spaces, do not know $T$, etc}


%\s{this paragraph here is crucial to the story. should be explained in more detail}
%\subsection{Inverse Reinforcement Learning with Regularization}

% \s{move the RL part in its subsection?}
Let us first consider imitation in Markov decision processes (as a special case to Markov games) and the framework of single-agent Maximum Entropy IRL
% \s{this is confusing. why suddenly single agent? it might be better to have clear separation between multi vs single agent stuff. otherwise this is going to be very confusing}\js{one way to make the transition is to just say we refer to single agent IRL as background, since RL has to precede IRL and we currently put RL with MARL}
\citep{ziebart2008maximum,ho2016generative}
where the goal is to recover a reward function $r$ that rationalizes the expert behavior $\pi_E$:
%which models expert behavior with high-entropy policies:
$$
\mb{IRL}(\pi_E) = \argmax_{r \in \bb{R}^{\mc{S} \times \mc{A}}} \bb{E}_{\pi_E}[r(s, a)] - \left(\max_{\pi \in \Pi} H(\pi) + \bb{E}_\pi[r(s, a)]\right)
$$
In practice, expectations with respect to $\pi_E$ are evaluated using samples from $\mc{D}$.
%In practice,  is unknown, and 
% We use ``imitation'' to describe the IRL approach for the remainder of this paper.

The IRL objective is ill-defined%\s{cite andrew's paper here}
~\citep{ng2000algorithms,finn2016guided} and there are often multiple valid solutions to the problem when we consider all $r \in \bb{R}^{\mc{S} \times \mc{A}}$. For example, we can assign the reward function for trajectories that are not visited by the expert arbitrarily so long as these trajectories yields lower rewards than the expert trajectories.
% \s{give an example?}
To resolve this ambiguity, \citet{ho2016generative} introduce a convex reward function regularizer $\psi: \bb{R}^{\mc{S} \times \mc{A}} \to \bb{R}$, which can be used to restrict rewards to be linear in a pre-determined set of features~\citep{ho2016generative}: 
%to select the most desirable reward function that explains the expert behavior:
\begin{gather}
\mb{IRL}_{\psi}(\pi_E) = \argmax_{r \in \bb{R}^{\mc{S} \times \mc{A}}}-\psi(r) + \bb{E}_{\pi_E}[r(s, a)] - \left(\max_{\pi \in \Pi} H(\pi) + \bb{E}_{\pi}[r(s, a)]\right) \label{eq:irl}
\end{gather}
% For example, $\psi$ can be used to restrict rewards to be linear in a pre-determined set of features~\citep{ho2016generative}.
%\s{this is an issue not specific to multi-agent. move to previous section? also cite the gail paper. not sure that's a standard way of viewing rl and irl.}

% In the remainder of the paper, we use $\mb{RL}(r)$ and $\mb{IRL}_\psi(\pi_E)$ to denote the ($H(\pi)$ and $\psi(r)$) regularized methods described above.

\subsection{Imitation by matching occupancy measures}
\cite{ho2016generative} interpret the imitation learning problem as matching two occupancy measures, i.e., the distribution over states and actions encountered when navigating the environment with a policy.
Formally, for a policy $\pi$, it is defined as $\rho_\piv(s, a) = \piv(a \vert s) \sum_{t=0}^{\infty} \gamma^t T(s_t = s \vert \pi)$. %This allows us to write $\bb{E}_\pi[r(s, a)] = \sum_{s, a} \rho_\piv(s, a) r(s, a)$ for any reward function $r$. 
%\citep{syed2008apprenticeship} showed that there is a one-to-one correspondence between policies and occupancy measures.
\cite{ho2016generative} draw a connection between IRL and occupancy measure matching, showing that the former is a dual of the latter:
\begin{prop}[Proposition 3.1 in \citep{ho2016generative}]
\label{thm:gail}
\normalfont 
$$\mb{RL} \circ \mb{IRL}_\psi(\pi_E) = \argmin_{\pi \in \Pi} -H(\pi) + \psi^\star(\rho_\pi - \rho_{\pi_E})$$
\end{prop}
% \s{make sure signs, max/min, and convexity/concavity are right here. signs are all swapped wrt to GAIL}
Here $\psi^\star(x) = \sup_{y} x^\top y - \psi(y)$ is the convex conjugate of $\psi$, which could be interpreted as a measure of similarity between the occupancy measures of expert policy and agent's policy. One instance of $\psi = \psi_{\text{GA}}$ gives rise to the Generative Adversarial Imitation Learning~(GAIL) method:
\begin{gather}
\psi^{\star}_{\text{GA}}(\rho_\pi - \rho_{\pi_E}) = \max_{D \in (0, 1)^{\mc{S} \times \mc{A}}} \bb{E}_{\pi_E}[\log(D(s, a))] + \bb{E}_{\pi}[\log (1 - D(s, a))] \label{eq:gaildisc}
\end{gather}
%The resulting imitation learning method corresponds to a two player minimax game~\citep{goodfellow2014generative}, where an adversary proposes a reward function, %that assigns lower rewards to policy trajectories and higher scores to expert ones, 
%while the agent aims to perform optimally under that reward function. 
The resulting imitation learning method from Proposition \ref{thm:gail} involves a \emph{discriminator} (a classifier $D$) competing with a \emph{generator} (a policy $\pi$). The discriminator attempts to distinguish real vs. synthetic trajectories (produced by $\pi$) by optimizing (\ref{eq:gaildisc}). The generator, on the other hand, aims to perform optimally under the reward function defined by the discriminator, %\s{which reward? clarify here}, 
thus ``fooling'' the discriminator with synthetic trajectories that are difficult to distinguish from the expert ones.
% \subsection{MARL}
% \js{I would argue we put this somewhere later than background section, as this also reflects our design choices}
% \begin{enumerate}
% \item what kind of policies? (history, markov, stationary)?
% \item optimality notions. existence of equilibria. uniqueness (some conditions in hu-wellman)
% \item what kind of multi-agent RL algorithm?
% \end{enumerate}
% The strategies that constitute a Nash
% equilibrium can be behavior strategies, Markov strategies,
% or stationary strategies. 

% Theorem 2 (Filar and Vrieze [4], Theorem 4.6.4)
% Every general-sum discounted stochastic game possesses at least one equilibrium point in \textbf{stationary} strategies. \textbf{check if holds for >2 players} \js{\citep{he2017stationary} has such a result}

% from Multiagent Reinforcement Learning: Theoretical Framework and an Algorithm


% incomplete but perfect information, meaning agents do not know
% other agents' payoffs functions but they can observe
% other agents' immediate payoffs and actions taken previously?





==> arXiv Submission/2_related.tex <==
% \section{Related work}
\section{Related work and discussion}
%\dl{could put background before related work?}\js{you think we should put related work after experiments?}
There is a vast literature on single-agent imitation learning~\citep{bagnell2015invitation}. 
%There are two major paradigms in imitation learning. 
Behavior Cloning~(BC) learns the policy through supervised learning~\citep{pomerleau1991efficient}. Inverse Reinforcement Learning (IRL) assumes the expert policy optimizes over some unknown reward, recovers the reward, and learns the policy through reinforcement learning (RL). 
BC does not require knowledge of transition probabilities or access to the environment, but suffers from compounding errors and covariate shift~\citep{ross2010efficient,ross2011reduction}.
%that affect generalization. 
% \begin{comment}
% IRL often require explicit knowledge of the transition probabilities~\citep{abbeel2004apprenticeship,syed2008apprenticeship} or black-box access to the environment~\citep{boularias2011relative,kalakrishnan2013learning,ho2016model,finn2016guided}. 
% \end{comment}
%\dl{word missing?}\js{not necessarily but i see your point} 
%It learns a reward function that could evaluate performance of other policies, but is expensive to run because it requires solving the RL problem in an inner learning loop.

Most existing work in multi-agent imitation learning assumes the agents have very specific reward structures. The most common case is fully cooperative agents, where the challenges mainly lie in other factors, such as unknown role assignments~\citep{le2017coordinated}, scalability to swarm systems~\citep{vsovsic2016inverse} and agents with partial observations~\citep{bogert2014multi}. In non-cooperative settings, ~\citet{lin2014multi} consider the case of IRL for two-player zero-sum games and cast the IRL problem as Bayesian inference, while~\citet{reddy2012inverse} assume agents are non-cooperative but the reward function is a linear combination of pre-specified features. 

Our work is the first to propose a general multi-agent IRL framework that bridges the gap between state-of-the art multi-agent reinforcement learning methods~\citep{lowe2017multi,foerster2016learning} and implicit generative models such as generative adversarial networks~\citep{goodfellow2014generative}. %\dl{what do you need adversarial training? Shouldn't you compare to them to show that?}\js{every thing is adversarial training; zero sum is just one type that does not match our current story}
Experimental results demonstrate that it is able to imitate complex behaviors in high-dimensional environments with both cooperative and adversarial interactions.
An interesting research direction is to explore new techniques for gathering expert demonstration; for example, when the expert is allowed to aid the agents by participating in part of the agent's learning process~\citep{hadfield2016cooperative}. 

==> arXiv Submission/3_methods.tex <==
\section{Generalizing IRL to Markov games}
\label{sec:mairl}

%Notable examples of $f(r)$ include \js{ng, abbeel, syed, zebart, ho}.

Extending imitation learning to multi-agent settings is difficult because there are multiple rewards (one for each agent) and the notion of optimality is complicated by the need to consider an equilibrium solution~\citep{hu1998multiagent}.
%In the case of Markov games, however, there are several problems for applying the IRL directly. In Markov games, agents could have different or even opposite goals. This makes it difficult to define a single reward function for all agents.
%Moreover, the environment is non-stationary for every agent because other agents might change their policies. Hence, the optimal policy of an agent depends on other agents. This requires us to consider other equilibrium concepts, such as Nash equilibrium~\citep{hu1998multiagent}.
We use $\mb{MARL}(r)$ to denote the set of (stationary and Markovian) policies that form a Nash equilibrium under $r$ and have the maximum %\s{maximum?} 
$\gamma$-discounted causal entropy (among all equilibria):
\begin{gather}
\mb{MARL}(\rv) = \argmin_{\piv \in \Pi, \vv \in \bb{R}^{\mc{S} \times N}} f_r(\piv, \vv) - H(\piv) \label{eq:real-marl} \\
v_i(s) \geq q_i(s, a_i) \quad \forall i \in [N], s \in \mc{S}, a_i \in \mc{A}_i \nonumber
\end{gather}
where $q$ is defined as in Eq.~\ref{eq:q}. Our goal is to define a suitable inverse operator MAIRL, in analogy to IRL in Eq. \ref{eq:irl}. The key idea of Eq. \ref{eq:irl} is to choose a reward that creates a \emph{margin} between the expert and every other policy. However, the \emph{constraints} in the Nash equilibrium optimization (Eq.~\ref{eq:real-marl}) can make this challenging.
%in Def. \ref{eq:real-marl} (defining a Nash equilibrium) make it difficult.
%to define a corresponding inverse optimization problem. 
% We therefore begin deriving
To that end, we derive an equivalent Lagrangian formulation of (\ref{eq:real-marl}), where we ``move'' the constraints into the objective function, so that we can define a margin between the expected reward of two sets of policies that captures their ``difference''. %\s{so that we can define a margin}
% \s{define as an argmin}
% \s{q as in eq xx}

\subsection{Equivalent constraints via temporal difference learning}

% Instead of having a unique solution (as in the case of $\mbox{RL}(r)$), a Markov game could have multiple Nash equilibria, i.e. $\mb{MARL}(r)$ can be a one-to-many relationship. If our goal is to find a specific Nash equilibrium, we can augment the constraints with the following proposition:
% \begin{prop}
% Assume $\pi^\star$ is some Nash equilibrium for reward $r$, and $\pi_i^\star$ is the unique optimal response to $\pi^\star_{-i}$ for all $i$.
% The following optimization problem has a unique optimal solution $\pi_i^\star$:
% \begin{gather}
%     \min_{\pi, v} f_r(\pi, v) \nonumber \\
%  \text{s.t.} \qquad  v_i(s) \geq \bb{E}_{\pi^\star_{-i}}[r_i(s, a) + \gamma \sum_{s' \in \mc{S}} T(s'|s, a) v_i(s')] \qquad \forall i, s, a, s' \nonumber
% \end{gather}
% \end{prop}

% \begin{comment}
% For any policy $\pi$, $f(\pi, \vh) = 0$ when $\vh$ is the value function of $\pi$ (due to Bellman equations). However, only policies that form a Nash equilibrium satisfies the constraints in Eq.~\ref{eq:marl}; we formalize this in the following Lemma.
% \begin{lemma}\label{thm:td1}
% %Define $\vh_i(s; \pi, r)$ as the value function for a set of policies $\pi$, which satisfies the Bellman equations (we use $\vh_i(s)$ to imply dependence over $\pi$ and $r$ for brevity):
% Let $\vh_i(s; \pi, r)$ be the solution to the Bellman equation
% %value function for a set of policies $\pi$:
% $$
% \vh_i(s; \pi, r) = \bb{E}_{\pi} [r_i(s, a) + \gamma \sum_{s' \in \mc{S}} T(s'|s, a) \vh_i(s')]
% $$
% and $\qh_i(s, a_i; \pi,r) = \bb{E}_{\pi_{-i}}[r_i(s, a) + \gamma \sum_{s' \in \mc{S}} T(s'|s, a) \vh_i(s'; \pi, r)]$. Then for any $\pi$,  $f_r(\pi, \vh(\pi)) = 0$. Furthermore, $\pi$ is Nash equilibrium under $r$ if and only if $\vh_i(s) \geq \qh_i(s, a_i)$ for all $i \in [N], s \in \mc{S}, a_i \in \mc{A}_i$.
% \end{lemma}
% \end{comment}

Intuitively, the Nash equilibrium constraints imply that any agent $i$ cannot improve $\pi_i$ 
%(or $v_i$) 
via 1-step temporal difference learning; if the condition for Equation~\ref{eq:q} is not satisfied for some $v_i$, $q_i$, and $(s, a_i)$, this would suggest that we can update the policy for agent $i$ and its value function.
% \s{expand this with an extra sentence, and refer to the equation. it might not be entirely obvious, so it's worth explaining more}
Based on this notion, we can derive equivalent versions of the constraints corresponding to $t$-step temporal difference (TD) learning.
\begin{theorem}
\label{thm:tdt}
For a certain policy $\piv$ and reward $\rv$, let $\vh_i(s; \piv, \rv)$ be the unique solution to the Bellman equation:
%value function for a set of policies $\pi$:
$$
\vh_i(s; \piv, \rv) = \bb{E}_{\pi} \left[r_i(s, \av) + \gamma \sum_{s' \in \mc{S}} T(s'|s, \av) \vh_i(s'; \piv, \rv)\right] \qquad \forall s \in \mc{S}
$$
% \s{is solution always guaranteed to exist? if so mention it}\js{yes, we assume the env is infinite horizon discounted cost, so the map should be a contraction}
% \s{since there is space, add dependency on the RHS}
% \s{not sure this is a bellman equation without the max}\js{it is just finding the value function, not obtaining the optimal value function}
% \s{add quantifiers over $s$, say this is for a certain policy and reward.}
% \s{again, bold fonts could help a lot here}
%Then for any $\pi$,  $f_r(\pi, \vh(\pi)) = 0$. Further, denote 
Denote $\qh_i^{(t)}(\{s^{(j)}, \av^{(j)}\}_{j=0}^{t-1}, s^{(t)}, a^{(t)}_i; \piv, \rv)$ as the discounted expected return for the $i$-th agent
%$\pi_i$ 
conditioned on visiting the trajectory $\{s^{(j)}, \av^{(j)}\}_{j=0}^{t-1}, s^{(t)}$ in the first $t-1$ steps and 
%$\pi_i$ 
choosing action $a^{(t)}_i$ at the $t$ step, when other agents use policy $\pi_{-i}$:% and $\pi_{-i}$ choosing action 
%\s{and $\pi_{-i}$}:
\begin{align*}
& \ \qh_i^{(t)}(\{s^{(j)}, \av^{(j)}\}_{j=0}^{t-1}, s^{(t)}, a^{(t)}_i; \piv, \rv)\\
=\ &\ \sum_{j=0}^{t-1} \gamma^{j} r_i(s^{(j)}, a^{(j)}) + \gamma^{t} \bb{E}_{\pi_{-i}}\left[r_i(s^{(t)}, \av^{(t)}) + \gamma \sum_{s' \in \mc{S}} T(s'|s, \av^{(t)}) \vh_i(s'; \piv, \rv)\right]
\end{align*}
% \s{add dependency on pi to qhat}
%where we define $\vh$ as in Lemma~\ref{thm:td1}.
Then $\pi$ is Nash equilibrium if and only if
\begin{gather}
    \vh_i(s^{(0)}; \piv, \rv) \geq \bb{E}_{\pi_{-i}}\left[\qh_i^{(t)}(\{s^{(j)}, \av^{(j)}\}_{j=0}^{t-1}, s^{(t)}, a^{(t)}_i; \piv, \rv)\right] \triangleq Q_i^{(t)}(\{s^{(j)}, a_i^{(j)}\}_{j=0}^{t}; \piv, \rv) \label{eq:bigq} \\
    \forall t \in \bb{N}^+, i \in [N], j \in [t], s^{(j)} \in \mc{S}, a^{(j)} \in \mc{A} \nonumber
\end{gather}
% \s{add dependency on pi in LHS}
\end{theorem}
% \s{you use a different = symbol for definitions before}
% \begin{proof}
% If $\pi$ is a Nash equilibrium, and at least one of the constraints does not hold, i.e. there exists some $i$ and $\{s^{(j)}, a_i^{(j)}\}_{j=0}^{t}$, such that
% $$\vh_i(s^{(0)}) < \bb{E}_{\pi_{-i}}[\qh_i^{(t)}(\{s^{(j)}, a^{(j)}\}_{j=0}^{t-1}, s^{(t)}, a^{(t)}_i)]$$
% Then agent $i$ can achieve a strictly higher expected return on its own if it chooses a particular sequence of actions by taking $a_i^{(j)}$ whenever it encounters state $s^{(j)}$, and following $\pi_i$ for the remaining states. We note that this is in expectation over the policy of other agents. Hence, we construct a policy for agent $i$ that has strictly higher value than $\pi_i$ without modifying $\pi_{-i}$, which contradicts the definition of Nash equilibrium.

% If the constraints hold, i.e for all $i$ and $\{s^{(j)}, a_i^{(j)}\}_{j=0}^{t}$,
% $$\vh_i(s^{(0)}) \geq \bb{E}_{\pi_{-i}}[\qh_i^{(t)}(\{s^{(j)}, a^{(j)}\}_{j=0}^{t-1}, s^{(t)}, a^{(t)}_i)]$$
% then we can construct any $\qh_i(s^{(0)}, a_i^{(0)})$ via a convex combination by taking the expectation over $\pi_i$:
% $$\qh_i(s^{(0)}, a_i^{(0)} = \bb{E}_{\pi_i}[\bb{E}_{\pi_{-i}}[\qh_i^{(t)}(\{s^{(j)}, a^{(j)}\}_{j=0}^{t-1}, s^{(t)}, a^{(t)}_i)]]$$
% where the expectation over $\pi_i$ is taken over actions $\{a_i^{(j)}\}_{j=0}^{t}$. Therefore, $\forall i, s, a_i$,
% $$
% \vh_i(s) \geq \qh_i(s, a_i)
% $$
% and we recover the constraints in Eq.~\ref{eq:marl}. By (\citep{prasad2015study}, Theorem 2.4), $\pi$ is a Nash equilibrium.
% \end{proof}
% \begin{theorem} \label{thm:tdt}
% Assume $\pi^\star$ is some Nash equilibrium for reward $r$, and $\forall i$, $\pi_i^\star$ is the unique optimal response to $\pi^\star_{-i}$. Let $\vh_i(s; \pi_\star)$ be the value function of agent $i$ with policy $\pi_i$ where the remaining agents use policy $\pi^\star_{-i}$.
% $\forall t \geq 0$, define $q_i^{(t)}(s^{(0)}, s^{(1)}, \ldots, s^{(t)}, a_i^{(0)}, a_i^{(1)}, \ldots, a_i^{(t)}; \pi^\star)$ as:
% $$
% \bb{E}_{\pi^\star_{-i}}[\sum_{j=0}^{t} \gamma^{j} r_i(s^{(j)}, a^{(j)}) + \gamma^{t+1} \sum_{s' \in \mc{S}} T(s'|s, a^{(t)}) \pi^\star_{-i}(a_{-i}^{(t)} | s^{(t)}) \vh_i(s'; \pi^\star) ]
% $$
% which is the expected discounted reward if agent $i$ had taken action sequence $(a_i^{(0)}, a_i^{(1)}, \ldots, a_i^{(t)})$ for states $(s^{(0)}, s^{(1)}, \ldots, s^{(t)})$ while other agents follow $\pi^{\star}_{-i}$. Then $\pi = \pi^\star$ is equivalent to
% \begin{gather}
%     \vh_i(s) \geq q_i^{(t)}(s^{(0)}, s^{(1)}, \ldots, s^{(t)}, a_i^{(0)}, a_i^{(1)}, \ldots, a_i^{(t)}; \pi^\star) \quad \forall i \in [N],  j \in [t], s_i^{(j)} \in \mc{S}, a_i^{(j)} \in \mc{A}_i. \nonumber %\label{eq:tdt}
% \end{gather}
% \end{theorem}
% \begin{proof}
% $\Rightarrow$: We have:
% \begin{align*}
%     \vh_i(s) &= \bb{E}_{s^{(1)}, a_i^{(1)}, \ldots, s^{(t)}, a_i^{(t)} \sim \pi_i}[\vh_i(s)] \\
%     &\geq \bb{E}_{s^{(1)}, a_i^{(1)}, \ldots, s^{(t)}, a_i^{(t)} \sim \pi_i}[q_i^{(t)}(s, s^{(1)}, \ldots, s^{(t)}, a_i, a_i^{(1)}, \ldots, a_i^{(t)})]  \\
%     & = \bb{E}_{\pi_{-i}^\star} [r_i(s, a) + \gamma \sum_{s' \in S} T(s'|s, a) \pi_{-i}^\star(a_{-i} | s) \vh(s')] \equiv q^\star(s, a_i)
% \end{align*}
% $\forall a_i \in \mc{A}_i$. Therefore, $\vh_i(s)$ is larger than convex combination of $q^\star(s, a_i)$, which includes the case of $\pi_i^\star$. Hence $\pi_i = \pi^\star_i$ since $\pi^\star_i$ is the unique optimal response to $\pi^\star_{-i}$. 

% $\Leftarrow$: If $\exists$ a sequence of states and actions for agent $i$ that violates the condition, then $\pi^\star_i$ is no longer the optimal response to $\pi^\star_{-i}$.
% % From Equation \ref{eq:td1} to \ref{eq:tdt} \js{need to think about it}: since
% % % we show this by induction. First, the statement is clearly true when $t=0$. Suppose that the statement is true for $t \in [0, k-1]$, we have:
% % \begin{align*}
% % q_i^{(t)}(s, s^{(1)}, \ldots, s^{(t)}, a_i, a_i^{(1)}, \ldots, a_i^{(k)}) & = \bb{E}_{\pi}[r_i(s, a_i) + \gamma q_i^{(k-1)}(s^{(1)}, a_i^{(1)}, \ldots, a_i^{(k)})] \\
% % & \leq \bb{E}_{\pi}[r_i(s, a_i) + \gamma \sum_{s' \in s} T(s'|s, a^{(t)}) v(s')] \\
% % & = q(s, a_i) \leq v(s)
% % \end{align*}
% % % Hence by induction the statement is true $\forall t \geq 0$.
% \end{proof}
Intuitively, Theorem~\ref{thm:tdt} states that if we replace the 1-step constraints with $(t+1)$-step constraints, we obtain the same solution as $\mb{MARL}(r)$, since $(t+1)$-step TD updates (over one agent at a time) is still stationary with respect to a Nash equilibrium solution. So the constraints can be unrolled for $t$ steps and rewritten as $\vh_i(s^{(0)}) \geq Q_i^{(t)}(\{s^{(j)}, a_i^{(j)}\}_{j=0}^{t}; \piv, \rv)$ (corresponding to Equation~\ref{eq:bigq}).
% \s{refer to equation where this is def (and give it a number)}

\subsection{Multi-agent inverse reinforcement learning}
We are now ready to construct the Lagrangian dual of the primal in Equation~\ref{eq:real-marl}, using the equivalent formulation from Theorem~\ref{thm:tdt}. The first observation is that for any policy $\piv$, $f(\piv, \vh) = 0$ when $\vh$ is defined as in Theorem~\ref{thm:tdt} (see Lemma~\ref{thm:td1} in appendix). Therefore, we only need to consider the ``unrolled'' constraints from Theorem~\ref{thm:tdt}, obtaining the following dual problem
%Consider the dual problem to the primal in Equation~\ref{eq:real-marl}  where we use $(t+1)$-step constraints and the value function for $\pi$:
\begin{align}
    \max_{\lambda \geq 0} \min_{\pi} L^{(t+1)}_\rv(\piv, \lambda) \triangleq \sum_{i = 1}^{N} \sum_{\tau_i \in \mc{T}_i^t} \lambda(\tau_i) \left(Q_i^{(t)}(\tau_i; \piv, \rv) - \vh_i(s^{(0)}; \piv, \rv)\right)
\end{align}
% \s{here it's important to show the dependencies on pi}
% \s{is there strong duality?}\js{no}
%\s{should it be v-Q?}
% \s{lambda}
% \s{vhat}
% \s{Q super}
% \s{add en English description for what this dual is}
where $\mc{T}_i(t)$ is the set of all length-$t$ trajectories of the form $\{s^{(j)}, a_i^{(j)}\}_{j=0}^{t}$, with $s^{(0)}$ as initial state, $\lambda$ is a vector of $N \cdot |\mc{T}_i(t)|$ Lagrange multipliers, and $\vh$ is defined as in 
Theorem~\ref{thm:tdt}. This dual formulation is a sum over agents and trajectories, which uniquely corresponds to the constraints in Equation \ref{eq:bigq}.
%Lemma~\ref{thm:td1}
%; hence $f_r(\pi, \vh(\pi))$ disappears because it is zero. 

In the following theorem, we show that for a specific choice of $\lambda$ we can recover the difference of the sum of expected rewards between two policies, a performance gap similar to the one used in single agent IRL in Eq. (\ref{eq:irl}). This amounts to ``relaxing'' the primal problem. 
%\js{so the issue is the choice of $\lambda$ depends on both $\pi$ and $\pi^\star$, and computes the probability where other agents is either $\pi$ or $\pi^\star$ (note we want to use it to represent some probability of trajectory). however, the expectation in $Q_i$ depends on $\pi$, so if we compare  $L(\pi)$ and $L(\pi^\star)$, we are using two sets of ``other agent policies'', which requires two sets of multiplers to make sense; the fix is simply remove one term}


\begin{theorem}\label{thm:dual}
For any two policies $\piv^\star$ and $\piv$, let 
$$\lambda^\star_\pi(\tau_i) = \eta(s^{(0)}) \pi_i(a_i^{(0)} | s^{(0)}) \prod_{j=1}^{t} \pi_i(a_i^{(j)} | s^{(j)}) \sum_{a_{-i}^{(j-1)}}T(s^{(j)} | s^{(j-1)}, a^{(j-1)}) \pi_{-i}^\star(a_{-i}^{(j)} | s^{(j)}) $$
%for all $\tau_i \in \mc{T}_i^t$
% \s{check subscripts}
be the probability of generating the sequence $\tau_i$ using policy $\pi_i$ and $\pi_{-i}^\star$. Then 
\begin{equation}
\lim_{t \to \infty} L_r^{(t+1)}(\piv^\star, \lambda^\star_\piv) = \sum_{i=1}^{N} \bb{E}_{\pi_i, \pi^\star_{-i}}[r_i(s,a)] - \sum_{i=1}^{N} \bb{E}_{\pi^\star_i, \pi^\star_{-i}}[r_i(s,a)] \label{eq:thm}
\end{equation}
where $L_r^{(t+1)}(\piv^\star, \lambda^\star_\pi)$ corresponds to the dual function where the multipliers are the probability of generating their respective trajectories of length $t$.
% \s{remind reader what L is}
\end{theorem}
%\s{add actions}
% \begin{proof}
% We use $Q^\star, \vh^\star$ to denote the quantities for policy $\pi^\star$.
% For the two terms in $L_r^{(t+1)}(\pi^\star, \lambda^\star)$ we have:
% \begin{align}
%     L_r^{(t+1)}(\pi^\star, \lambda^\star) = \sum_{i = 1}^{N} \sum_{\tau_i \in \mc{T}_i} \lambda^\star(\tau_i) (Q_i^\star(\tau_i) - \vh_i^\star(s^{(0)})) \label{eq:gap}
% \end{align}
% For any agent $i$, we note that 
% $$\sum_{\tau_i \in \mc{T}_i} \lambda^\star(\tau_i) Q_i^\star(\tau_i) = \bb{E}_{\pi_i} \bb{E}_{\pi^\star_{-i}} [\sum_{j=0}^{t-1} \gamma^j r_i(s^{(j)}, a^{(j)})] + \gamma^t \qh_i^\star(s^{t}, a_i^{(t)})]$$
% which amounts to using $\pi_i$ for agent $i$ for the first $t$ steps and using $\pi^\star_i$ for the remaining steps, whereas other agents follow $\pi^\star_{-i}$. As $t \to \infty$, this converges to $\bb{E}_{\pi_i, \pi^\star_{-i}}[r_i]$ since $\gamma^t \to 0$ and $q^\star_i(s^{(t)}, a_u^{(t)})$ is bounded. Moreover, for $\vh^\star_i(s^{(0)}$, we have
% $$
% \sum_{\tau_i \in \mc{T}_i} \lambda^\star(\tau_i) \vh^\star_i(s^{(0)}) = \bb{E}_{s^{(0)} \sim \eta}[v_i(s^{(0)})] = \bb{E}_{\pi^\star}[r_i]
% $$
% Combining the two we have $L_r^{(t+1)}(\pi^\star, \lambda^\star) = \sum_{i=1}^{N} \bb{E}_{\pi_i, \pi^\star_{-i}}[r_i] - \sum_{i=1}^{N} \bb{E}_{\pi^\star}[r_i]$, and we can substitute $\pi^\star$ to get $L_r^{(t+1)}(\pi^\star, \lambda^\star) = 0$, which finishes the proof.
% \end{proof}

We provide a proof in Appendix~\ref{app:dual}. Intuitively, the $\lambda^\star(\tau_i)$ weights correspond to the probability of generating trajectory $\tau_i$ when the policy is $\pi_i$ for agent $i$ and $\pi_{-i}^\star$ for the other agents. As $t \to \infty$, the first term of left hand side in Equation~\ref{eq:thm}, $\sum_{i = 1}^{N} \sum_{\tau_i \in \mc{T}_i^t} \lambda(\tau_i) Q_i^{(t)}(\tau_i)$, converges to the expected total reward  $\bb{E}_{\pi_i, \pi_{-i}^\star}[r_i]$, which is the first term of right hand side. The marginal of $\lambda^\star$ over the initial states is the initial state distribution, so the second term of left hand side, $\sum_{s} \vh(s) \eta(s)$, converges to $\bb{E}_{\pi^\star_i, \pi^\star_{-i}}[r_i]$, which is the second term of right hand side. Thus, the left hand side and right hand side of Equation~\ref{eq:thm} are the same as $t \to \infty$. %\s{this paragraph is not clear}

Theorem \ref{thm:dual} motivates the following definition of multi-agent IRL with regularizer $\psi$.
%Let us assume that our expert policy $\pi_E$ forms a Nash equilibrium under some reward function $r$; and that for each agent $i$, $\pi_{E_i}$ is the unique optimal response to other experts $\pi_{E_{-i}}$ \s{where do we use this assumption?}. 
%Therefore, if we substitute $\pi^\star$ with $\pi_E$ in the right hand side for Equation~\ref{eq:gap}, this basically measures the difference in expected rewards between $\pi_i$ and $\pi_{E_i}$ when other agents adopt policy $\pi_{E_{-i}}$. 
%We consider the following definition of $\mb{MAIRL}$ with regularizer $\psi$:
\begin{align}
    \mb{MAIRL}_{\psi}(\piv_E) = \argmax_{\rv} -\psi(\rv) + \sum_{i=1}^{N} (\bb{E}_{\piv_E}[r_i]) - \left(\max_\piv \sum_{i=1}^{N} (\beta H_i(\pi_i) +  \bb{E}_{\pi_i, \pi_{E_{-i}}}[r_i]) \right),
\end{align}
where $H_i(\pi_i) = \bb{E}_{\pi_i, \pi_{E_{-i}}}[-\log \pi_i(a_i | s)]$ 
% \s{missing log?}
is the discounted causal entropy for policy $\pi_i$ when other agents follow $\pi_{E_{-i}}$, and $\beta$ is a hyper-parameter controlling the strength of the entropy regularization term as in~\citep{ho2016generative}. This formulation is a strict generalization to the single agent IRL in~\citep{ho2016generative}.
\begin{corollary}
If $N = 1$, $\beta=1$ then {\normalfont $\mb{MAIRL}_\psi(\piv_E) = \mb{IRL}_\psi(\piv_E)$}.
\end{corollary}
% Furthermore, let us assume that $\psi(r) = \sum_{i=1}^{N} \psi_i(r_i)$, i.e. the regularization on different agent's reward functions can be separated:
% \begin{align}
%     \mb{MAIRL}_{\psi}(\pi_E) = \argmax_{r} \sum_{i=1}^{N} \psi_i(r_i) + \bb{E}_{\pi_E}[r_i] - (\max_{\pi_i} H_i(\pi_i) + \bb{E}_{\pi_i, \pi_{E_{-i}}}[r_i])
% \end{align}
% We can now invoke Proposition~\ref{thm:gail} for each $i$.
Furthermore, if the regularization $\psi$ is additively separable, and for each agent $i$, $\pi_{E_i}$ is the unique optimal response to other experts $\pi_{E_{-i}}$, we obtain the following:
%on different agent's reward functions can be separated,
%we can invoke Proposition~\ref{thm:gail} for each $i$.
\begin{theorem}\label{thm:om}
Assume that $\psi(\rv) = \sum_{i=1}^{N} \psi_i(r_i)$, $\psi_i$ is convex for each $i \in [N]$, 
% \s{do we need concavity/convexity on psi?}
and that {\normalfont $\mb{MARL}(r)$} has a unique solution\footnote{The set of Nash equilibria is not always convex, so we have to assume $\mb{MARL}(r)$ returns a unique solution.} for all {\normalfont $r \in \mb{MAIRL}_\psi (\pi_E)$}, then {\normalfont
$$\mb{MARL} \circ \mb{MAIRL}_\psi (\pi_E) = \argmin_{\pi \in \Pi} \sum_{i=1}^{N} -\beta H_i(\pi_i) + \psi_i^\star(\rho_{\pi_{i, E_{-i}}} - \rho_{\pi_{E}})$$ }
where $\pi_{i, E_{-i}}$ denotes $\pi_i$ for agent $i$ and $\pi_{E_{-i}}$ for other agents.
\end{theorem}
% \s{change assumptiob}
% \begin{proof}
% Define the ``MARL'' objective for a single agent $i$ where other agents have policy $\pi_{E_i}$:
% $$
% \mb{MARL}_i(r_i) = \max_{\pi_i} H_i(\pi_i) + \bb{E}_{\pi_i, \pi_{E_{-i}}}[r_i]
% $$
% Define the ``MAIRL'' objective for a single agent $i$ where other agents have policy $\pi_E$:
% $$
% \mb{MAIRL}_{i, \psi}(\pi^\star) = \argmax_{r_i} \psi_i(r_i) + \bb{E}_{\pi_E}[r_i] - (\max_{\pi_i} H_i(\pi_i) + \bb{E}_{\pi_i, \pi_{E_{-i}}}[r_i])
% $$
% Since $r_i$ and $\pi_i$'s are independent in the $\mb{MAIRL}$ objective, the solution to $\mb{MAIRL}_\psi$ can be represented by the solutions of $\mb{MAIRL}_{i, \psi}$ for each $i$:
% $$
% \mb{MAIRL}_\psi = [\mb{MAIRL}_{1, \psi}, \ldots, \mb{MAIRL}_{N, \psi}]
% $$
% Moreover, the single agent ``MARL'' objective $\mb{MARL}_i(r_i)$ has a unique solution $\pi_{E_i}$, which also composes the (unique) solution to $\mb{MARL}$ (which we assumed in Section~\ref{sec:mairl}. Therefore, 
% $$
% \mb{MARL}(r) = [\mb{MARL}_1(r_1), \ldots, \mb{MARL}_N(r_N)]
% $$
% So we can use Proposition 3.1 in~\cite{ho2016generative} for each agent $i$ with $\mb{MARL}_i(r_i)$ and $\mb{MAIRL}_{i, \psi}(\pi^\star)$ and achieve the same solution as $\mb{MARL} \circ \mb{MAIRL}_\psi$.
% \end{proof}

% \js{we need to think of MARL definition here, currently does not seem to break but the connection is not super close}
The above theorem suggests that $\psi$-regularized multi-agent inverse reinforcement learning is seeking, for each agent $i$, a policy whose occupancy measure is close to one where we replace policy $\pi_i$ with expert $\pi_{E_i}$, as measured by the convex function $\psi_i^\star$.

However, we do not assume access to the expert policy $\pi_E$ during training, so it is not possible to obtain $\rho_{\pi_{i, E_{-i}}}$. In the settings of this paper, we consider an alternative approach where we match the occupancy measure between $\rho_{\pi_E}$ and $\rho_{\pi}$ instead. We can obtain our practical algorithm if we select an adversarial reward function regularizer and remove the effect from entropy regularizers.
\begin{prop}\label{thm:magail}
If $\beta=0$, and $\psi(\rv) = \sum_{i=1}^{N} \psi_{i}(r_i)$ where $\psi_{i}(r_i) = \bb{E}_{\pi_E}[g(r_i)]$ if $r_i > 0$; $+\infty$ otherwise, and $$
g(x) = \left\{
                \begin{array}{ll}
                  -x - \log (1 - e^x) & \text{if}\quad r_i > 0\\
                 +\infty & \text{otherwise}\\
                \end{array} \right.
$$
then
$$
\argmin_\pi \sum_{i=1}^{N} \psi_{i}^\star (\rho_{\pi_i, \pi_{E_{-i}}} - \rho_{\pi_E}) = \argmin_\pi \sum_{i=1}^{N} \psi_{i}^\star (\rho_{\pi_i,\pi_{-i}} - \rho_{\pi_E}) = \pi_E
$$
% \s{use a bracket to define g, this is hard to read}
\end{prop}
Theorem~\ref{thm:om} and Proposition~\ref{thm:magail} discuss the differences from the single agent scenario. On the one hand, in Theorem~\ref{thm:om} we make the assumption that $\mb{MARL}(\rv)$ has a unique solution, which is always true in the single agent case due to convexity of the space of the optimal policies. On the other hand, in Proposition~\ref{thm:magail} we remove the entropy regularizer because here the causal entropy for $\pi_i$ may depend on the policies of the other agents, so the entropy regularizer on two sides are not the same quantity. Specifically, the entropy for the left hand side conditions on $\pi_{E_{-i}}$ and the entropy for the right hand side conditions on $\pi_{-i}$ (which would disappear in the single-agent case).
%  \js{need to think more} \s{add a bit of high level discussion of what is going on here. basically, discuss what's different from single agent case, and what we had to change. nonconvexity, use a bound, etc.}

% \begin{proof}\js{super sloppy, but for the interest of time; at least i think there is no issues to the proof}
% Let us first consider $\argmin_{\pi} \sum_{i=1}^{N} -H_i(\pi_i) + \psi_i^\star(\pi_{i, E_{-i}} - \rho_{\pi_E})$. 
% For each agent $i$, define $\bar{L}(\rho, r) = - H_i(\rho) - \sum_{s, a} r_i(s, a) (\rho_{\pi_i}(s, a) - \rho_{\pi_E}(s, a))$, where $\rho_{\pi_E}$ is the occupancy measure obtained by all agents using $\pi_E$ and $\rho_{\pi_i}$ is the occupancy measure obtained by agents using $\pi_{E_{-i}}$ and $\pi_{i}$. Given that $\psi_i$ is a constant function, we have the following due to Lemma 3.3 in~\cite{ho2016generative}:
% \begin{align*}
%     \tilde{r_i} \in \mb{MAIRL}_{\psi_i}(\pi_E) & = \argmax_{r \in \bb{R}^{\mc{S} \times \mc{A}}} + \bb{E}_{\pi_{E_i}, \pi_i}[r_i] - \bb{E}_{\pi}[r_i] + \text{const} \\
%     & = \argmax_{r \in \bb{R}^{\mc{S} \times \mc{A}}} \min_{\rho} - \bar{H}(\rho) - \sum_{s, a} r_i(s, a) (\rho_{\pi_i}(s, a) - \rho_{\pi_{E_i}}(s, a)) \\
%     & = \argmax_{r \in \bb{R}^{\mc{S} \times \mc{A}}} \min_{\rho} \bar{L}(\rho, r)
% \end{align*}
% Using the strong duality argument similar to Proposition 3.2 in~\cite{ho2016generative}, this implies that the solution $\rho_{\pi_i} = \rho_{\pi_E}$ for all $i$ (note that this is conditioned on other agents being $\pi_{E_{-i}}$. A similar argument holds for $\argmin_{\pi} \sum_{i=1}^{N} -\hat{H}_i(\pi_i) + \psi_i^\star(\rho_{\pi_i} - \rho_{\pi_E})$, so both values are equal to $\pi_E$.
% \end{proof}


% \begin{proof}
% First, the expectation of value functions over $\eta(s)$ is the expected return:
% $$\sum_{s^{(0)} \in \mc{S}} \eta(s^{(0)}) \vh_i(s^{(0)}) = \bb{E}_\pi[r_i]$$

% Then, $q$ is the  

% For $L^{(t+1)}_r(\pi^\star, \hat{\lambda)}$, we have:
% $$
% L^{(t+1)}_r(\pi^\star, \hat{\lambda}) = \sum_{S_t \in \mc{S}^{t+1}} \sum_{A_t \in \mc{A}^{t+1}} \sum_{i =1}^{N} \lambda(S_t, A_t, i) (q_i^{(t)}(S_t, A_t; \pi^\star) - \vh_i(s^{(0)}))
% $$
% \end{proof}

% For any choice of positive multiplier function $\lambda$, $\pi$ is Nash under $r$ is equivalent to $L_r(\pi, \lambda)$ is zero, so we are allowed to choose any positive multiplier function that ``smoothes'' the objective and still keep Nash equilibrium policies as the global optimum. In particular, we show in the following theorem, that 

% if $\pi \in \mb{MARL}(r)$, then $(\pi, v)$ is a globally optimal solutions for the constrained optimization problem in Equation~\ref{eq:marl}, where $v$ is the value function of $\pi$. In fact, $f(\pi, v) = 0$ is always true when $v$ is the value function of $\pi$; however, only policies that form a Nash equilibrium do not violate the constraints, which implies that we are not able to update $\pi$ or $v$ for a single agent via temporal difference learning (TD(1)).

% \js{maybe cut we can change the definition}
% \begin{gather}
% \mb{MARL}(r) = \argmin_{\pi \in \Pi} \min_{v \in \bb{R}^{\mc{S}}} f_r(\pi, v) \\
% \text{s.t.} \quad v_i(s) \geq q_i(s, a_i) \quad \forall i \in [1, N], s \in \mc{S}, a_i \in \mc{A}_i \nonumber
% \end{gather}
%\subsection{Finding Nash Equilibria with RL}
% We assume that in Multi-Agent IRL (MAIRL), the experts form a Nash equilibrium under a certain reward function that we wish to recover. In the following sections, we formalize this problem, draw connections between Multi-Agent RL and Nash equilibrium, and provide practical algorithms that performs efficient MAIRL. \js{we have not formalized the problem yet...}
%\s{this section could be moved into the RL one 3.2. it kind of breaks the flow here}\js{wouldnt that make prelim too long? also this sort of contains our assumption (that RL can solve NE problems) or we can just move this paragraph}
 %\s{maybe briefly summarize conditions under which they exist}\js{I couldn't understand a thing about their condition (only that it is pretty general)... and conditions by other papers seem too sparse}

% Moreover, we assume that $\pi_i(a_i \vert o_i) > 0, \forall \pi_i \in \Pi_i, a_i \in \mc{A}_i, o_i \in \mc{O}_i$, i.e. all actions are possible at any state. This is a mild assumption for policy gradients since actions are often sampled from Gaussian or through softmax functions. Therefore, when agents reach an Nash equilibrium, the policy gradient for each agent is zero (because we avoid boundary conditions). \s{can we justify why we make this assumption? intuitively at least?} \js{1. that gradient = 0 for all agents represents all NE (i thought this is the intuition?); 2. easier for arguing existence stationary distribution in GAN theorem}

% The process of finding a Nash equilibrium can be defined as a constrained optimization problem~\citep{filar2012competitive}. We slightly abuse notations in RL, and let $Q_i(s, \pi)$ be the Q-function for agent $i$ by selecting the stochastic policy $\pi_i$ when other agents select $\pi_{-i}$, and $V_i(s, \pi_{-i})$ be the value function of $i$ (by taking expectation over $\pi_i(a \vert o)$). The objective is then~\footnote{We assume we need to find $V$ and $Q$ (a function of $V$ and $r$) through dynamic programming in the process.}:
% \begin{gather}
% \min_{\pi \in \Pi, V} f_r(\pi, V) = \sum_{i=1}^{N} \left(\sum_{s \in \mc{S}} V_i(s, \pi_{-i}) - Q_i(s, \pi) \right) \label{eq:marl} \\
% V_i(s, \pi_{-i}) \geq Q_i(s, \hat{\pi_i}, \pi_{-i}) \quad \forall i, s, \hat{\pi}_i \label{eq:marl-condition} %i \in [1, N], s \in \mc{S}, \hat{\pi}_i \in \Pi_i 
% \end{gather}
% \s{wrap this into a definition of MARL. its a key concept and we want reader to pay attention}
% whose global minimum is zero; $\pi$ form a Nash equilibrium if and only if $f_r(\pi, V)$ reaches zero while being a feasible solution. Intuitively, this problem requires each agent to find the best response to other agents' policies. 

% Solving the problem in Eq.~\ref{eq:marl} is complicated by the fact that these constraints are non-convex. In general MGs, gradient methods can converge to a local minimum but not the global minimum~\citep{prasad2015study} and hence convergence to a Nash equilibrium is not guaranteed. While one could use concepts such as $\epsilon$-Nash equilibrium for local optima~\citep{filar2012competitive}, we assume RL methods can converge to Nash equilibria for ease of exposition in this paper and let $\mb{MARL}(r)$ be the set of policies that are globally optimal to the objective in Eq.~\ref{eq:marl}:
% \begin{gather}
% \mb{MARL}(r) = \argmin_{\pi \in \Pi} \min_{V \in \bb{R}^{\mc{S}}} f_r(\pi, V) \\
% \text{s.t.} \quad V_i(s) \geq Q_i(s, a_i) \quad \forall i \in [1, N], s \in \mc{S}, a_i \in \mc{A}_i \nonumber
% \end{gather}
% \s{fix this as in the previous def, make sure all domains are specified}
% \js{can write the entire process formally as a constrained optimization problem with non-convex constraints not sure if this could explain the connections between OMs}

% \js{introduce $v$ $q$ functions and objective as $\min_{\pi, v} f(\pi, v)$ with non-convex contraints}

% \js{although there are no direct conclusions as to actor critic converges to a NE; I guess then we should talk for two cases, cooperative (converges to NE), non-cooperative (does not converge to NE but converges to a KKT point)}
% \subsection{Multi-Agent Inverse Reinforcement Learning}
% \label{sec:mairl}
% Instead of having a unique solution (as in the case of $\mbox{RL}(r)$), 
% a Markov game could have multiple Nash equilibria, i.e. $\mb{MARL}(r)$ can be a one-to-many relationship.
% A simple example would be the stateless coordination game, where two agents can select from three actions and receive a reward of $1$ if they select the same action. Two policies form a Nash equilibrium if they both assign 0.5 probability to the same two actions, so there are at least three Nash equilibria.%Two policies form a Nash equilibrium as long as both agents use the same mixed strategy. 
% % \s{is this true? is $1/3$ , $1/3$ a NE?}.
% % \s{if an agent does $1/3,2/3$, then i'm incentivized to always choose the second action ($0,1$)?}\js{changed to 3 actions, where you can have 3 (0.5, 0.5)}

% While one reward could lead to multiple equilibrium solutions, $\pi_E$ should always be an element of the set under a reasonable definition for multi-agent inverse reinforcement learning. 
% Formally, we define $\mb{MAIRL}(\pi_E)$ as the set of reward functions under which experts form a Nash equilibrium:
% \begin{gather}
% \mb{MAIRL}(\pi_E) = \{ r \vert \pi_E \in \mb{MARL}(r) \}
% \end{gather}
% or equivalently using the definition in Equation~\ref{eq:marl} (recall that minimizing $f_r(\pi, v)$ under feasibility constraints is equivalent to finding a Nash equilibrium):
% \begin{gather}
% \mb{MAIRL}(\pi_E) = \argmin_{r, v} f_r(\pi_E, v) \\
% \text{s.t.} \quad v_i(s) \geq q_i(s, a_i) \quad \forall i \in [1, N], s \in \mc{S}, a_i \in \mc{A}_i \nonumber
% \end{gather}
% It is easy to verify the following (proof in Appendix~\ref{app:convex}):
% \begin{prop}
% \label{thm:convex}
% {\normalfont $\mb{MAIRL}(\pi_E)$} is convex.
% \end{prop}
% %\s{might be good to add an extra sentece at the end of the proof, explaining why you can use those inequalities and why the conclusion follows}
% % We can also introduce a (convex) reward function regularizer $\psi: \bb{R}^{\mc{S} \times \mc{A}} \to \bb{R}$ to specify our prior over the (unknown) reward:
% % \begin{gather}
% % \mb{MAIRL}_\psi(\pi_E) = \argmin_{r, v} f_r(\pi_E, v) + \psi(r) \\
% % \text{s.t.} \quad V_i(s) \geq q_i(s, a_i) \quad \forall i \in [1, N], s \in \mc{S}, a_i \in \mc{A}_i \nonumber
% % \end{gather}
% \js{remove MAIRL reg}


% \subsection{Formalizing Multi-Agent Imitation}
% \label{sec:mairl-def}
% The imitation learning process for a single agent can be described as finding $\pi \in \mb{RL} \circ \mb{IRL}_{\psi}(\pi_E)$; one would be tempted to describe the multi-agent imitation process as finding a reward under which the experts form a Nash equilibrium (through a suitable $\mb{MAIRL}_{\psi}(\pi_E)$ operator), and then recover the policy by solving the corresponding MARL problem, i.e. finding $\pi \in \mb{MARL} \circ \mb{MAIRL}_{\psi}(\pi_E)$.
% %where $\mb{MAIRL}$ can be defined in a similar fashion to $\mb{IRL}_\psi$. 
% However, this notion is problematic in multi-agent scenarios. In the coordination game, even if the IRL process recovers the true reward (under which the expert is a Nash equilibrium), the MARL process could still lead to equilibrium behaviors that deviate significantly from the demonstrations. 
% We illustrate this in Figure~\ref{fig:mairl} (left).

% %\s{Again, double check this}

%  % Note that this is not an issue for single-agent IRL because $\mb{RL}(r)$ is an injection; all reward functions recovered by $\mb{IRL}_{\psi}(\pi_E)$ have a single optimal policy. \s{again, not sure this is true. see above.}

% % \s{move mairl definition to previous section. this section mixes irl and imitiation and this is confusing. mairl is a concept needed in this section, so it should be defined before}
% Our definition to multi-agent imitation has to take this into account.
% This suggests the following informal definition:
% \begin{quote}
% Finding policies that form a Nash equilibrium under \textit{all} the reward functions under which the experts also form a Nash equilibrium.
% \end{quote}
% Formally, we define the multi-agent imitation process $\mb{MIM}(\pi_E)$ as:
% % \s{confusing}
% % which implies the following objective:
% %\s{should/can we add a psi regularizer over $r$ in here?}
% \begin{align}
% & \argmin_{\pi \in \Pi} \min_{v \in \bb{R}^{\mc{S}}} \max_{r \in \bb{R}^{\mc{S} \times \mc{A}}} f_r(\pi, v) \label{eq:mim}\\
% \text{s.t.}& \quad v_i(s) \geq q_i(s, a_i) \quad \forall i \in [1, N], s \in \mc{S}, a_i \in \mc{A}_i \nonumber \\
% \text{and}& \quad r \in \mb{MAIRL}(\pi_E) \nonumber
% \end{align}
% which is equivalent to:
% \begin{gather}
% \mb{MIM}(\pi_E) = \bigcap_{r \in \text{MAIRL}(\pi_E)} \mb{MARL}(r) \label{eq:cap}
% \end{gather}
% \begin{prop}
% \label{thm:equiv}
% Eq. (\ref{eq:mim}) and (\ref{eq:cap}) are equivalent definitions of $\mb{MIM}(\pi_E)$.
% % for { \normalfont $\mb{MIM}(\pi_E)$}.
% \end{prop}
% We prove the equivalence in Appendix~\ref{app:equiv}.
% % \s{proof seems ok}
% % \begin{proof} We show that each equation implies the other:
% % \begin{description}
% % \item[\ref{eq:mim} $\Rightarrow$ \ref{eq:cap}] Since $\pi_E$ is a globally optimal solution to Equation~\ref{eq:mim}, the optimal value of Equation~\ref{eq:mim} is zero. If $\pi$ is a solution to Equation~\ref{eq:mim} then $\min_V f_r(\pi, V) = 0$ holds true for all feasible $r \in \mb{MAIRL}(\pi_E)$. Hence $\pi$ is an element of $\mb{MARL}(r)$ for all $r \in \mb{MAIRL}(\pi_E)$ and an element of their intersection.
% % \item[\ref{eq:cap} $\Rightarrow$ \ref{eq:mim}] If $\pi$ is an element of $\mb{MIM}(\pi_E)$, then for all $r \in \mb{MAIRL}(\pi_E)$, $\pi \in \mb{MARL}(r)$ and $\min_V f_r(\pi, V) = 0$ (for feasible $V$), so $\pi$ is a globally optimal solution to Equation~\ref{eq:mim} with objective value zero.
% % \end{description}
% % Hence the two definitions to $\mb{MIM}(\pi_E)$ are equivalent.
% % \end{proof}
% % \s{is it easy to prove this equivalence? add a proof}
% % \s{so MIM is also convex?}\js{not necessarily? since MARL is not?}
% %Assuming the expert policy is the only solution to Eq.~\ref{eq:mairl}, they will eventually reach $\pi_E$. \s{why is this a reasonable assumption?}
% % \s{this convexity property should also be moved in the mairl subsection}
% %
% %% commenting out for now to save space. both daniel and i got confused reading this so might be better to cut..

% % The process of solving Equation (\ref{eq:mim}) by alternating maximization and minimization can be interpreted as having two players competing with each other: one player proposes a policy $\pi$ 
% % %(non-repeatedly) 
% % that minimizes $f_r(\pi, V)$ under some reward function $r$, while the other player proposes another reward function $r' \in \mb{MAIRL}(\pi_E)$ under which $f_{r'}(\pi, V) > 0$. 
% % The process stops when an element in $\mb{MIM}(\pi_E)$ has been selected by the first player. \dl{could put a summarh of the section at the beginning to say what you're showing and how you do it; this is hard to follow}

% %\s{not clear what the 'process'  is, we haven't really said how we solve that minimax problem}\js{i aimed to say a very high-level argument; in this case we can assume they are just  oracles?}
% %We illustrate this process in Figure~\ref{fig:mairl} (left).

% % \begin{figure}
% % \centering
% % \begin{subfigure}[b]{0.23\textwidth}
% % \includegraphics[width=\textwidth]{figs/mairl}
% % \end{subfigure}
% % ~
% % \begin{subfigure}[b]{0.23\textwidth}
% % \includegraphics[width=\textwidth]{figs/magail}
% % \end{subfigure}
% % \caption{Left: in Markov games, one reward function could have several Nash equilibria and $\pi_E$ is always one of them. Right: occupancy measure matching allows the learned policy to converge to the expert by using a surrogate of the imitation objective, which gives rise to multi-agent GAIL.} %\js{change figures to mairl}}
% % \label{fig:mairl}
% % \end{figure}

% \subsection{Multi-Agent Imitation by Matching Occupancy Measures}
% \label{sec:3.3}

% As before, we can incorporate a reward regularizer $\psi$ into $\mb{MIM}(\pi_E)$ as follows:
% \begin{gather}
% \mb{MIM}_\psi(\pi_E) = \argmax_{\pi \in \Pi} \max_{v} \min_{r \in \bb{R}^{\mc{S} \times \mc{A}}} \mc{L}_\psi(\pi_E, v) \nonumber\\
% \mc{L}_\psi(\pi_E, v) = - f_r(\pi, v) + f_r(\pi_E, v) + \psi(r) \nonumber \\
% r \in \mb{MAIRL}(\pi_E)\nonumber
% \end{gather}
% % \s{missing constraints}
% % \s{looks like there's a swapped max-min}\js{yes how should we address this?} \s{is it a typo? i thought max over V should be outside} \js{yes but if we switch this the global optimal is unchanged? it makes it easier to write $L_\psi$}\s{are you on slack?}
% where we negate %\dl{not the right word; invert $= f^{-1}$} 
% $f_r(\pi, v)$ to convert the mini-max problem in~(\ref{eq:mim}) to a max-min one, and use the fact that $\min_V f_r(\pi_E, v) = 0$ for all $r \in \mb{MAIRL}(\pi_E)$. 

% Notice that by definition~(\ref{eq:marl}), $f_r(\pi_E, v)$ is defined as a sum of components $\sum v_i(s) - q_i(s, a_i)$, where each term $v_i(s) - q_i(s, a_i)$ is non-negative when the constraints in~(\ref{eq:marl}) are satisfied.
% %\s{what are these components?} 
% Therefore, if we multiply each term by a non-negative coefficient, the global optimum (which is a Nash equilibrium under feasibility constraints) will not change. By choosing a suitable weighting, we introduce a surrogate to $\mc{L}_\psi(\pi_E, v)$ defined in terms of expected rewards which is much easier to estimate and optimize (an in a standard RL).
% %draw a connection between $f_r(\pi, V)$ and expected rewards, which allows us to utilize difference in expected reward (which is much easier to compute and optimize over) as a surrogate to $\mc{L}_\psi(\pi_E, V)$.
% % \s{explain the various changes made here. this sentence is disconnected}

% \begin{theorem}
% \label{thm:ub}
% Assume that the support of the initial state distribution $\eta(s)$ is $\mc{S}$, $\pi_i(a_i \vert s) > 0$ for all $i \in [1, N], a_i \in \mc{A}_i$, and the transition matrix $T$ is ergodic.
% Let $\mc{R} \subset \bb{R}^{\mc{S} \times \mc{A}}$ be the set of reward functions such that $\forall r \in \mc{R}$, %\js{i dont think i need this; only $\pi_E$ is optimal Nash}
% \begin{gather}
% \pi_{E_i} = \argmax_{\pi_i \in \Pi_i} \bb{E}_{\pi_i, \pi_{-i}}[r_i(s, a)] \label{eq:expert-best}
% \end{gather}
% and $\pi_{E_i}$ is the only optimal policy. Let 
% \begin{gather}
% f_r^w(\pi, v) = \sum_{i=1}^{N} \Bigg(\sum_{s \in \mc{S}, a_i \in \mc{A}_i} w_i(s, a_i) \Big(v_i(s) - q_i(s, a_i)\Big) \Bigg)
% \nonumber
% \end{gather}
% where $w_i(s, a_i) = \eta(s)\pi_i(a_i \vert s)$.
% If $f_r(\pi_E, v)$ is a valid solution to Eq.~\ref{eq:marl}, then
% \begin{gather}
% f_r^w(\pi, v) - f_r^w(\pi_E, v) \leq \sum_{i=1}^{N} (\bb{E}_{\pi_E}[r_i] -\bb{E}_{\pi}[r_i]) 
% \label{eq:surrogate}
% %\nonumber
% \end{gather}
% for all $r \in \mc{R}$.
% \end{theorem}
% \begin{proof}
% In Appendix~\ref{app:ub}.
% \end{proof}
% This suggests that the difference in expected returns  between the expert and the policy (the RHS of Eq. (\ref{eq:surrogate})) can be utilized to bound $\mc{L}_\psi(\pi_E)$ for a specific set of reward functions $\mc{R}$ for which the expert is the only Nash equilibrium. %(for example, a feasible element in $\mc{R}$ is simply $\mb{KL}(\pi_E \Vert \pi_i)$). \dl{put intuition first, it's hard to parse at first}\dl{choosing $\mathcal{R}$ seems crucial, can you give any intuition?} 
% We can then use this as a surrogate  to the original $\mb{MIM}(\pi_E)$ objective:
% \begin{gather}
% \sum_{i=1}^{N} (\bb{E}_{\pi}[r_i] -\bb{E}_{\pi_E}[r_i]) + \psi(r) \leq L_\psi^w(\pi_E, v)
% \end{gather}
% where $\mc{L}_\psi^w(\pi_E, v) = - f_r^w(\pi, v) + f_r^w(\pi_E, v) + \psi(r)$.

% Let us assume that $\psi(r) = \sum_{i=1}^{N} \psi_i(r_i)$, i.e. the regularization on different agent's reward functions are independent. 
% We obtain $\mb{MIM}^\star_\psi(\pi_E)$ which is a surrogate to $\mb{MIM}_\psi(\pi_E)$:
% \begin{gather}
% \argmax_{\pi \in \Pi} \min_{r \in \bb{R}^{\mc{S} \times \mc{A}}} \sum_{i=1}^{N} (\bb{E}_\pi[r_i] -\bb{E}_{\pi_E}[r_i]) + \psi_i(r_i) \nonumber
% \end{gather}
% %Since $\pi_i$ and $\psi_i$ are independent, this amounts to optimizing several independent IRL problems.
% Proposition~\ref{thm:gail} implies that this is equivalent to matching the occupancy measure for each individual agent as measured by $\psi_i^\star$ respectively:
% \begin{gather}
% \mb{MIM}^\star_\psi(\pi_E) = \argmin_{\pi \in \Pi} \sum_{i=1}^{N} \psi_i^\star(\rho_i - \rho_{E_i}) \label{eq:mim-gail}
% \end{gather}
% where $\psi^\star$ is the convex conjugate of $\psi$. Hence, matching occupancy measures between the policies and the expert can be viewed as a surrogate objective to multi-agent imitation.

% % \s{i suspect you can prove an analogous of theorem Theorem 2 of Syed et al. [29]. given occuancy measure, you can work out all the policies by marginalizing. and viceversa}

% In a distributed setting, we can let each agent $i$ imitate the expert by trying to match its own occupancy measure $\rho_{\pi_i}(s, a_i) = \pi_i(a_i \vert s) \sum_{t=0}^{\infty} \gamma^t T(s_t = s \vert \pi)$ with the corresponding occupancy measure of the $i$-th expert $\rho_{\pi_{E_i}}(s, a_i) = \pi_{E_i}(a_i \vert s) \sum_{t=0}^{\infty} \gamma^t T(s_t = s \vert \pi_E)$ according to $\psi^\star_i$. 
% Intuitively, if each agent manages to match their own occupancy measure, then the joint policy of all agents will match the occupancy measure of the expert. We show the following and prove it in Appendix~\ref{app:tv}.

% % \s{another thing probably true is that you can bound the variation of the joint in terms of the sum of variations on the marginals of the agents. then we optimize for this bound, which is a reasonable thing to do and does not require assumptions}
% \begin{prop}
% \label{thm:tv}
% If $\rho_{\pi_i}$ converges to $\rho_{\pi_{E_i}}$ in total variation for all $i$, then $\rho_{\pi}$ converges to $\rho_{\pi_E}$ in total variation.
% \end{prop}


% Moreover, occupancy measures and policies also have one-to-one correspondence in the multi-agent setting, so this process can recover the expert policy.
% \begin{prop}

% \end{prop}

% \s{a more intuitive argument is that if $\rho_{\pi_i}(s, a) = \rho_{\pi_E}(s, a)$, then $\rho_{\pi_i}(a|s) = \rho_{\pi_E}(a|s)$ which means you have gotten the the right policy for every agent (and therefore the joint must match)?}

% However, multi-agent imitation is no longer strictly the dual of the occupancy measure matching problem due to non-convexity.

%\s{maybe some of this stuff should go in background, so that there's a clear separation between old and new stuff}


% It is possible, though, to decrease the probability of learning an undesirable policy by obtaining multiple solutions to the MAIRL problem and choose one set of policies that is the equilibrium of some of the corresponding reward functions, i.e. find $\pi$ such that $\pi \in \mb{MARL}(r), \forall r \in \mb{MAIRL}(\pi_E)$.  %\js{can we prove some formal statement?}

% We address this problem by interpreting the imitation learning problem as matching two distributions~\citep{ho2016generative}: the occupancy measure of the expert policy and that of the learned policy. 

% For a policy $\pi$, define its occupancy measure $\rho_\pi: \mc{S} \times \mc{A} \to \bb{R}$ as $\rho_\pi(s, a) = \pi(a \vert o) \sum_{t=0}^{\infty} \gamma^t T(s_t = s \vert \pi)$. This allows us to write $\bb{E}_\pi[r(s, a)] = \sum_{s, a} \rho_\pi(s, a) r(s, a)$ for any reward function $r$. \citet{syed2008apprenticeship} showed that there is a one-to-one correspondence between policies and occupancy measures.

% First, as Hu and Wellman (Hu Wellman, 1998)
% note, the concept of optimality, central to MDPs, must be replaced with an equilibrium
% solution concept, such as the Nash equilibrium. Second, the non-uniqueness of equilibria
% means that in MIRL, in addition to multiple reasonable solutions for a given inversion
% model, there may be multiple inversion models that are all equally sensible approaches to
% solving the problem \js{I saw this bit; but saying this at the front may make this look simple; i wanted to push this to the reviewers who know more in deep learning and single agent rl than MARL}

% \subsection{Inverse Reinforcement Learning for Multiple Agents}
% \s{what are the inputs?
% sequences of state action pairs $s,...$,environment (black box),...}
% \s{what is the output?}
% \s{need to be clear about what is known and not. dynamics? (no, implicit via samples). discount factor? etc. }


% One such concept is the Nash equilibrium. 

% \js{define mixed NE and cite some theory: mixed strategy NE exists when finite players finite actions; Nash equilibrium exists if the set of choices is compact with continuous payoff. these assumptions are reasonable in practical RL cases, so we assume NE always exists}

% Hence, we informally characterize IRL in Markov games (Multi-Agent IRL) as the process of finding a set of reward functions, one for each agent, under which the set of expert policies $\{\pi_{E_1}, \ldots, \pi_{E_N}\}$ is a Nash equilibrium.
% This leads to the following objective:
% \begin{gather}
% \min_{r_1, \ldots, r_N} f(r_1, \ldots, r_N) \\
% \text{s.t} \quad \pi_{E_i} = \argmax_{\pi_i} \bb{E}_{\pi_{E_{-i}}, \pi_i}[r_i(s, a)] \quad \forall i \in [1, N]\nonumber
% \end{gather}
% where we learn a set of reward functions $\{r_i\}_{i=1}^{N}$

% \s{we might want to sell this as multi-agent imitation/apprenticeship learning}

% \s{define an RL operator, and IRL operator and imitation as RL(IRL(data))}
% \subsection{\js{some section title}}







==> arXiv Submission/4_practical.tex <==
\section{Practical multi-agent imitation learning}
%\s{it all makes sense up until sec 3.3, then the remaining part seems disconnected.}
\definecolor{disc}{cmyk}{0.60, 0.0, 0.60, 0.20}
\definecolor{expert}{cmyk}{0.70, 0.15, 0.00, 0.20}
\definecolor{policy}{cmyk}{0.0, 0.45, 0.60, 0.20}
\definecolor{env}{cmyk}{0.30, 0.60, 0.00, 0.20}


Despite the recent successes in deep RL, it is notoriously hard to train policies with RL algorithms%\s{an RL algorithm is not something you train} 
because of high variance gradient estimates. This is further exacerbated in Markov games since an agent's optimal policy depends on other agents~\citep{lowe2017multi,foerster2016learning}.
% Moreover, the imitation procedure defined in Equation~\ref{eq:cap} is not tractable since it requires computing all solutions in $\mb{MAIRL}(\pi_E)$ and then obtaining all solutions to $\mb{MARL}(r)$. 
In this section, we address these problems and propose practical algorithms for multi-agent imitation. % that optimizes the surrogate occupancy measure matching objective $\mb{MIM}^\star_\psi(\pi_E)$ in Equation~(\ref{eq:mim-gail}).

\subsection{Multi-agent generative adversarial imitation learning}
%\s{start saying which of the various optimization problems we are trying to solve. refer to equation}
% Interestingly, this corresponds well to the two-player game introduced in Generative Adversarial Imitation Learning (GAIL,~\citet{ho2016generative}): the policy (generator) aims to perform well under the reward given by the discriminator, which tries to assign high reward to expert trajectories and low reward to agent ones. 

% We notice that this process is strikingly similar to the one proposed by Eq.~\ref{eq:mairl}, which is also a two player game between the reward function and the policy. \js{we might want to expand this bit} 
We select $\psi_i$ to be our reward function regularizer in Proposition~\ref{thm:magail}; 
% \s{this GA stuff is not defined..refer back to proposition 6?}
this corresponds to the two-player game introduced in Generative Adversarial Imitation Learning (GAIL,~\citep{ho2016generative}).
%, as well as the altering maximization and minimization for $\mb{MIM}(\pi_E)$ in Equation~\ref{eq:mim}. 
%\s{i don't think players alternate. that's how we solve it..}
For each agent $i$, we have a discriminator (denoted as $D_{\omega_i}$) mapping state action-pairs to \emph{scores} optimized to discriminate expert demonstrations from behaviors produced by $\pi_i$. Implicitly, $D_{\omega_i}$ plays the role of a reward function for the generator, which in turn attempts to train the agent to maximize its reward thus fooling the discriminator. We optimize the following objective:
\begin{gather}
\min_\theta \max_{\omega}\mathbb{E}_{\piv_\theta}\left[\sum_{i=1}^{N} \log D_{\omega_i}(s, a_i)\right] + \mathbb{E}_{\piv_E}\left[\sum_{i=1}^{N} \log (1 - D_{\omega_i}(s, a_i))\right] \label{eq:magail:adv}
\end{gather}
%This process is similar to coordinate descent in the sense that each agent updates their policies independently. %\dl{maybe say this still converges to the right thing because of Thm 1 and Prop 4?}\js{i tried to prove it in thm 2 (commented below) but stefano says we wont risk it (since the proof might be handwavy} 
We update $\pi_\theta$ through reinforcement learning, where we also use a baseline $V_\phi$ to reduce variance.
We outline the algorithm -- Multi-Agent GAIL (MAGAIL) -- in Appendix~\ref{app:magail}.%~\ref{alg:magail}.
% In the following theorem, we show that this allows the agents to converge to their respective expert policies.
% \begin{theorem}
% Assume the transition matrix $T$ is ergodic and $\pi_i(a_i \vert s) > 0$ for all $i \in [1, N], a_i \in \mc{A}_i, s \in \mc{S}$. Assume $\pi_i$ and $D_i$ have enough capacity to represent any function. At each step we successively allow the discriminator to reach its optimum given $\pi$ and update $\pi_i$ so as to improve the criterion with sufficiently small updates
% $$
% U_i = \bb{E}_{\pi_E}[\log D_i(s, a_i)] + \bb{E}_{\pi}[\log (1 - D_i(s, a_i))]
% $$
% then $\pi_i$ converges to $\pi_{E_i}$ for all $i$. 
% \label{thm:mairl}
% \end{theorem}
% \begin{proof}
% In Appendix~\ref{app:mairl}.
% \end{proof}
% \s{dont think i understand the proof..} \js{mostly by joining the proof in ian goodfellow's gan paper and coordinate descent; there he proved that gan objective is convex w.r.t the generated distribution $p_g$ and then using small steps to update leads to global optimal; here I use that argument and (handwavyly) say gan objective is convex in $\pi_i$ so $\pi_i$ can optimize its own objective and move closer to $\pi_E$; other agents optimize their own objective and also move closer to their expert although not optimizing the same function as $i$; if no $\pi_i$ moves then it must be global optimum.}
% Since $T$ is ergodic and $\pi$ assigns positive probability to all actions, the Markov chain defined by $T$, $\pi$ and initial state distribution $\eta(s)$ has a stationary distribution, say $P(s)$. Hence for each agent we are trying to match $P_E(s)\pi_E(a_i \vert s)$ with $g_i = P(s)\pi_i(a_i \vert s)$. Similar to the argument in \citep{goodfellow2014generative}, $U_i$ is convex and differentiable in $g_i$ and so is $\sup_{D_i} U_i$. The difference in our case is that we are only allowed to affect $g_i$ through one coordinate $\pi_i$ ($\pi_i$ can be viewed as a coordinate because $\{\pi_i\}_{i=1}^{N}$ are independent and $g_i$ is a function of $\pi$, $T$ is stationary). If we update $\pi_i$ with sufficiently small updates that improves $U_i$ then $\pi_i$ will not move away from $\pi_{E_i}$ (under the metric induced by Jensen-Shannon divergence), since $U_i$ is also convex and differentiable in the coordinate of $\pi_i$.

% We then show by contradiction that at each step at least one $\pi_i$ could improve unless ``global'' optimum is reached at $\pi = \pi_E$. Suppose at some point $\pi \neq \pi_E$, all $\pi_i$ ceased to update; then from Theorem 1 in~\citep{goodfellow2014generative}, all $D_i$ are confused and $P(s) \pi(a_i \vert s) = P_E(s) \pi_E(a_i \vert s)$, and subsequently $P(s) = P_E(s)$ and $\pi(a_i \vert s) = \pi_E(a_i \vert s)$ for all $s \in \mc{S}, a_i \in \mc{A}_i, i \in [1, N]$. This implies that $\rho(\pi) = \rho(\pi_E)$, which contradicts $\pi \neq \pi_E$ since policies and occupancy measures have one-to-one correspondence~\citep{syed2008apprenticeship}. 

% Hence for each $U_i$, the process corresponds to coordinate descent over a  convex and differentiable function, where at least one of $\pi_i$ and $\pi_{-i}$ will improve. This process converges to the global optimum~\citep{nesterov2012efficiency}.
%and slowly to converge to the global optimum. Since agent are not necessarily optimizing the same reward, the assumption about slow policy updates is crucial to the proof.
% \s{algorithm uses a $V_\phi$ which is undefined..need to discuss what it is, add to inputs, etc.}
% \s{dynamics do not have the observations} \js{you mean MG? $\ov$ is is a function that maps states to observation}

% \begin{algorithm}[h]
%   \caption{Multi-Agent GAIL (MAGAIL)}
%   \label{alg:magail}
% \begin{algorithmic}
%   \STATE {\bfseries Input:} Initial parameters of policies,  discriminators and value~(baseline) estimators $\theta_0, \omega_0$, $\phi_0$; expert trajectories $\mc{D} = \{(s_j, a_j)\}_{j=0}^{M}$; batch size $B$; Markov game as a black box $(N, \mc{S}, \mc{A}, \eta, T, r, \ov, \gamma)$.
%   \STATE \textbf{Output: } Learned policies $\pi_\theta$ and reward functions $D_\omega$.
%   \FOR{$u=0, 1, 2, \ldots $}
%       \STATE Obtain trajectories of size $B$ from $\pi$ by the process: $s_0 \sim \eta(s), a_t \sim \pi_{\theta_u}(a_t \vert s_t), s_{t+1} \sim T(s_t \vert a_t)$.
%       \STATE Sample state-action pairs from $\mc{D}$ with batch size $B$.
%       \STATE Denote state-action pairs from $\pi$ and $\mc{D}$ as $\chi$ and $\chi_E$.
% 		\FOR{$i = 1, \ldots, n$}
%       \STATE Update $\omega_{i}$ to increase the objective
%       \vspace{-0.5em}$$\mathbb{E}_{\chi}[\log D_{\omega_i}(s, a_i)] + \mathbb{E}_{\chi_E}[\log (1 - D_{\omega_i}(s, a_i))]$$
%       \STATE Compute value estimate $V^\star$ and advantage estimate $A_i$ for $(s, a) \in \chi$.
%       \STATE Update $\phi_i$ to decrease the objective
%       \vspace{-0.5em}$$\mathbb{E}_{\chi}[(V_\phi(s, a_{-i}) - V^\star(s, a_{-i}))^2] $$
%       \STATE Update $\theta_i$ by policy gradient with small step sizes:
%       \vspace{-0.5em}$$\mathbb{E}_{\chi}[\nabla_{\theta_i} \pi_{\theta_i}(a_i \vert o_i) A_i(s, a)]$$
%       \ENDFOR
%   \ENDFOR
% \end{algorithmic}
% \end{algorithm}

%\dl{what is $\chi$?}\js{in alg 1. Denote state action pairs...}
% \paragraph{Interpretation}
% \s{not sure this section is understandable..}
% Multi-agent GAIL seems to propose a reward and train the corresponding policy iteratively; the fact that it manages to converge to the expert seems to contradict with our argument about $\mb{MARL}(r)$ being non-injective in Section~\ref{sec:mairl}, which suggests that training the policy over a learned reward could deviate from expert behavior.

% The major difference is that the policy proposals cannot be selected freely. In fact, they are restricted to ones that are close to the previous proposal, since $\pi$ are being changed using small gradient steps. Since the expert policy $\pi_E$ achieves $f_r(\pi, V)=0$ for all valid $r$, the policy proposer will have to choose policies close to $\pi_E$ in order to maximize its payoff. 
% From another perspective, we decrease the probability of learning an undesirable policy by proposing multiple solutions to the MAIRL problem and choose one $\pi$ that minimizes $f_r(\pi, V)$ for the corresponding reward functions. 
% This interpretation is illustrated in Figure~\ref{fig:mairl} (right).

% \subsection{Assumptions over Reward Structure}
We can augment the reward regularizer $\psi(r)$ using an indicator $y(r)$ denoting whether $r$ fits our prior knowledge; the augmented reward regularizer $\hat{\psi}: \bb{R}^{\mc{S} \times \mc{A}} \to \bb{R} \cup \{\infty\}$ is then: $\psi(r)$ if $y(r) = 1$ and $\infty$ if $y(r) = 0$.
% $$
% \hat{\psi}(r) = 
% \begin{cases}
% \psi(r) & \text{if} \quad y(r) = 1\\
% \infty & \text{if} \quad y(r) = 0\\
% \end{cases}
% $$
%
%This naturally excludes all reward functions that do not fit our prior. 
%
%Moreover, $\hat{\psi}(r)$ is convex so long as the set $\{r \vert y(r) = 1\}$ is convex. 
We introduce three types of $y(r)$ for common settings.

\paragraph{Centralized} The easiest case is to assume that the agents are fully cooperative, i.e. they share the same reward function. Here $y(r) = \bb{I}(r_1 = r_2 = \ldots r_n)$ and $\psi(r) = \psi_{\text{GA}}(r)$. One could argue this corresponds to the GAIL case, where the RL procedure operates on multiple agents (a joint policy). %, so conclusions in~\citep{ho2016generative} would still hold. %\js{so conclusions in GAIL paper still holds here}

\paragraph{Decentralized} We make no prior assumptions over the correlation between the rewards. %, yet we assume experts are acting rationally under a reward function that depends only on its own observations and actions. 
Here $y(r) = \bb{I}(r_i \in \bb{R}^{\mc{O}_i \times \mc{A}_i})$ and $\psi_i(r_i) = \psi_{\text{GA}}(r_i)$. This corresponds to one discriminator for each agent which discriminates the trajectories as observed by agent $i$. However, these discriminators are not learned independently as they interact indirectly via the environment. %\s{reward should be a function of state not observation?} \js{yes but in this case we use observation as input to discrminiantor; how should we define the set ?}

\paragraph{Zero Sum} Assume there are two agents that receive opposite rewards, so $r_1 = -r_2$. 
As such, $\psi$ is no longer additively separable.
%This assumption does not directly fit into our IRL framework because $\psi_i(r_i)$ are no longer independent. 
%\dl{I understood the first thing not the last thing}\js{removed; not important} 
Nevertheless, an adversarial training procedure can be designed using the following fact:
\begin{gather}
v(\pi_{E_1}, \pi_2) \geq v(\pi_{E_1}, \pi_{E_2}) \geq v(\pi_1, \pi_{E_2}) \nonumber
\end{gather}
where $v(\pi_1, \pi_2) = \bb{E}_{\pi_1, \pi_2}[r_1(s, a)]$ is the expected outcome for agent 1. The discriminator could maximize the reward for trajectories in $(\pi_{E_1}, \pi_2)$ and minimize the reward for trajectories in $(\pi_2, \pi_{E_1})$.
%\dl{I see the intution, maybe could be made more rigorous?}\js{maybe if i had more time i could say sth like the 4.4 argument...}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.30\linewidth}
    \includegraphics[width=\textwidth]{figs/cent.pdf}
    \caption{Centralized (Cooperative)}
    \end{subfigure}
    ~
    \begin{subfigure}{0.30\linewidth}
    \includegraphics[width=\textwidth]{figs/decent.pdf}
    \caption{Decentralized (Mixed)}
    \end{subfigure}
    ~
    \begin{subfigure}{0.30\linewidth}
    \includegraphics[width=\textwidth]{figs/zsum.pdf}
    \caption{Zero-sum (Competitive)}
    \end{subfigure}
    \caption{Different MAGAIL algorithms obtained with different priors on the reward structure. The \textcolor{disc}{discriminator} tries to assign higher rewards to top row and low rewards to bottom row. In centralized and decentralized, the \textcolor{policy}{policy} operates with the \textcolor{env}{environment} to match the \textcolor{expert}{expert} rewards. In zero-sum, the \textcolor{policy}{policy} do not interact with the \textcolor{env}{environment}; \textcolor{expert}{expert} and \textcolor{policy}{policy} trajectories are paired together as input to the \textcolor{disc}{discriminator}.}
    \label{fig:priors}
\end{figure}
These three settings are in summarized in Figure \ref{fig:priors}.
\subsection{Multi-agent actor-critic with Kronecker factors}
To optimize over the generator parameters $\theta$ in Eq. (\ref{eq:magail:adv})
%Once we obtain rewards from the discriminators, %proposal $r \in \mb{MAIRL}_\psi(\pi_E)$, 
we wish to use an algorithm for multi-agent RL that has good sample efficiency in practice. 
Our algorithm, which we refer to as Multi-agent Actor-Critic with Kronecker-factors (MACK), is based on Actor-Critic with Kronecker-factored Trust Region (ACKTR,~\citep{wu2017scalable}), a state-of-the-art natural policy gradient~\citep{amari1998natural,kakade2002natural} method in deep RL. %ACKTR approximates the Fisher matrix with the Kronecker product of smaller matrices (K-FAC, ~\citep{martens2015optimizing}), which allows it to perform efficient approximate natural policy gradient updates. \js{maybe cut} % This has allowed ACKTR to have better sample complexity 
%than its gradient descent counterpart
% in a range of tasks~\citep{mnih2016asynchronous} .
MACK uses the framework of centralized training with decentralized execution~\citep{foerster2016learning}; policies are trained with additional information to reduce variance but such information is not used during execution time. 
%In particular, 
We let the advantage function of every agent agent be a function of all agents' observations and actions:
\begin{align}
A_{\phi_i}^{\pi_{i}}(s, a_t) = \sum_{j=0}^{k-1} &(\gamma^j r(s_{t+j}, a_{t+j}) + \gamma^k V_{\phi_i}^{\pi_i}(s_{t+k}, a_{-i, t})) V_{\phi_i}^{\pi_i}(s_{t}, a_{-i, t})
\end{align}
where $V_{\phi_i}^{\pi_i}(s_k, a_{-i})$ is the baseline for $i$, utilizing the additional information $(a_{-i})$ for variance reduction. % treats other agents as a part of the environment, whereas 
%  serves as additional information for variance reduction. 
% The policy gradient for agent $i$ is written as:
% $$
% \nabla_\theta R_i(\theta_i) = \bb{E}_\pi \big[\sum_{t=0}^{T} \nabla_\theta \pi_{\theta_i}(a_{i, t} \vert o_{i, t}) A_{\theta_i}^{\pi_i}(o_t, a_t) \big]
%$$
We use (approximated) natural policy gradients to update both $\theta$ and $\phi$ but without trust regions to schedule the learning rate -- a linear decay learning rate schedule achieves similar empirical performance.

MACK has some notable differences from Multi-Agent Deep Deterministic Policy Gradient~\citep{lowe2017multi}. On the one hand, MACK does not assume knowledge of other agent's policies nor tries to infer them; the value estimator merely collects experience from other agents (and treats them as black boxes). On the other hand, MACK does not require gradient estimators such as Gumbel-softmax~\citep{jang2016categorical,maddison2016concrete} to optimize over discrete actions, which is necessary for DDPG~\citep{lillicrap2015continuous}. %\dl{are you sure that's true? I thought you only needed likelihood}\js{\citep{lowe2017multi} said so -- i think you need to take gradient wrt actions because deterministic policies? (or use gumbel)}

==> arXiv Submission/5_experiments.tex <==
\section{Experiments}
We evaluate the performance of (centralized, decentralized, and zero-sum versions) of MAGAIL under two types of environments. One is a particle environment which allows for complex interactions and behaviors; the other is a control task, where multiple agents try to cooperate and move a plank forward. We collect results by averaging over 5 random seeds. Our implementation is based on OpenAI baselines~\citep{baselines}; please refer to Appendix~\ref{app:exps} for implementation details. %We will release our code upon publication.

We compare our methods (centralized, decentralized, zero-sum MAGAIL) with two baselines. The first is behavior cloning (BC), which learns a maximum likelihood estimate for $a_i$ given each state $s$ and does not require actions from other agents. The second baseline is the GAIL IRL baseline that operates on each agent separately -- for each agent we first pretrain the other agents with BC, and then train the agent with GAIL; we then gather the trained GAIL policies from all the agents and evaluate their performance.

\subsection{Particle environments}
% \begin{figure*}[h]
% \centering
% \includegraphics[width=\textwidth]{figs/new_compe}
% \caption{Normalized agent performance in competitive environments. If the adversary is BC (first and third charts), higher performance is better; if agent is BC, lower performance is better (second and fourth charts).}
% \label{fig:adversary}
% \end{figure*}

We first consider the particle environment proposed in~\citep{lowe2017multi},
which consists of several agents and landmarks. %Agents may take \emph{physical actions} and \emph{communication actions} that get broadcasted to other agents. 
We consider two cooperative environments and two competitive ones. All environments have an underlying true reward function that allows us to evaluate the performance of learned agents. 

The environments include: \textbf{Cooperative Communication} -- two agents must cooperate to reach one of three colored landmarks. One agent (``speaker'') knows the goal but cannot move, so it must convey the message to the other agent (``listener'') that moves but does not observe the goal. \textbf{Cooperative Navigation} -- three agents must cooperate through physical actions to reach three landmarks; ideally, each agent should cover a single landmark. \textbf{Keep-Away} -- two agents have contradictory goals, where agent 1 tries to reach one of the two targeted landmarks, while agent 2 (the adversary) tries to keep agent 1 from reaching its target. The adversary does not observe the target, so it must act based on agent 1's actions. \textbf{Predator-Prey} -- three slower cooperating adversaries must chase the faster agent in a randomly generated environment with obstacles; the adversaries are rewarded by touching the agent while the agent is penalized.

For the cooperative tasks, we use an analytic expression defining the expert policy; for the competitive tasks, we use MACK to train expert policies based on the true underlying rewards (using larger policy and value networks than the ones that we use for imitation). We then use the expert policies to simulate trajectories $\mathcal{D}$, and then do imitation learning on $\mathcal{D}$ as demonstrations, where we assume the underlying rewards are unknown. %, nor is the expert policy. 
Following~\citep{li17infogail}, we pretrain our Multi-Agent GAIL methods and the GAIL baseline using behavior cloning as initialization to reduce sample complexity for exploration. We consider 100 to 400 episodes of expert demonstrations, each with 50 timesteps, which is close to the amount of timesteps used for the control tasks in~\cite{ho2016generative}. Moreover, we randomly sample the starting position of agent and landmarks each episode, so our policies have to learn to generalize when they encounter new settings.

\subsubsection{Cooperative tasks}
We evaluate performance in cooperative tasks via the average expected reward obtained by all the agents in an episode. In this environment, the starting state is randomly initialized, so generalization is crucial. We do not consider the zero-sum case, since it violates the cooperative nature of the task.
We display the performance of centralized, decentralized, GAIL and BC in Figure~\ref{fig:comp}.


Naturally, the performance of BC and MAGAIL increases with more expert demonstrations. MAGAIL performs consistently better than BC in all the settings; interestingly, in the cooperative communication task, centralized MAGAIL is able to achieve expert-level performance with only 200 demonstrations, but BC fails to come close even with 400 trajectories. Moreover, the centralized MAGAIL performs slightly better than decentralized MAGAIL due to the better prior, but decentralized MAGAIL still learns a highly correlated reward between two agents. % Cooperative MAGAIL also has slightly better sample complexity as shown in Figure~\ref{fig:coop}.

\begin{figure}
\centering
\includegraphics[width=\textwidth]{figs/cooperative_result}
\caption{Average true reward from cooperative tasks. Performance of experts and random policies are normalized to one and zero respectively. We use inverse log scale for better comparison.}
\label{fig:comp}
\end{figure}

\begin{table}
\centering
\caption{Average agent rewards in competitive tasks. We compare behavior cloning (BC), GAIL (G), Centralized (C), Decentralized (D), and Zero-Sum (ZS) methods. Best marked in bold (high vs. low rewards is preferable depending on the agent vs. adversary role).
}
\begin{tabular}{c|ccccc|cccc}
\hline
  Task  &  \multicolumn{9}{c}{Predator-Prey}\\\hline
    Agent  & \multicolumn{5}{c|}{Behavior Cloning} & G & C & D & ZS\\
    Adversary & BC & G & C & D & ZS & \multicolumn{4}{c}{Behavior Cloning} \\\hline
    Rewards & -93.20 & -93.71 & -93.75 & -95.22 & \textbf{-95.48} & -90.55 & -91.36 & \textbf{-85.00} & -89.4 \\\hline
    \hline
    Task  &  \multicolumn{9}{c}{Keep-Away}\\\hline
    Agent  & \multicolumn{5}{c|}{Behavior Cloning} & G & C & D & ZS\\
    Adversary & BC & G & C & D & ZS & \multicolumn{4}{c}{Behavior Cloning} \\\hline
    Rewards & 24.22 & 24.04 & 23.28 & 23.56 & \textbf{23.19} & 26.22 & 26.61 & \textbf{28.73} & 27.80 \\\hline
\end{tabular}
\label{tab:competitive}
\end{table}

% \begin{figure}
% \centering
% \includegraphics[width=0.45\textwidth]{figs/new_comple}
% \caption{Sample complexity of multi-agent GAIL methods under cooperative tasks. Performance of experts is normalized to one, and performance of behavior cloning is normalized to zero. The standard deviation is computed with respect to episodes, and is noisy due to randomness in the environment.}
% \label{fig:coop}
% \end{figure}

\subsubsection{Competitive tasks}
We consider all three types of Multi-Agent GAIL (centralized, decentralized, zero-sum) and BC in both competitive tasks. Since there are two opposing sides, it is hard to measure performance directly. Therefore, we compare by letting (agents trained by) BC play against (adversaries trained by) other methods, and vice versa.
%fixing one side of the agents to be BC and their adversaries as other methods. 
From Table~\ref{tab:competitive}, decentralized and zero-sum MAGAIL often perform better than centralized MAGAIL and BC, which suggests that the selection of the suitable prior $\hat{\psi}$ is important for good empirical performance. More details for all the particle environments are in the appendix. 

\subsection{Cooperative control}
In some cases we are presented with sub-optimal expert demonstrations because the environment has changed; we consider this case in a cooperative control task~\citep{madrl}, where $N$ bipedal walkers cooperate to move a long plank forward; the agents have incentive to collaborate since the plank is much longer than any of the agents. The expert demonstrates its policy on an environment with no bumps on the ground and heavy weights, while we perform imitation in an new environment with bumps and lighter weights
%only $10\%$ of heavy weight; 
(so one is likely to use too much force). Agents trained with BC tend to act more aggressively and fail, whereas agents trained with centralized MAGAIL can adapt to the new environment. With 10 (imperfect) expert demonstrations, BC agents have a chance of failure of $39.8\%$ (with a reward of 1.26), while centralized MAGAIL agents fail only $26.2\%$ of the time (with a reward of 26.57). We show videos of respective policies in the supplementary.
% \s{add video of this in supplementary}
% \js{getting results; only want to say number due to space limitations}
% \js{bc is already good but GAIL can work better with imperfect demonstrations and env distributional shift}\dl{looks weird to not be a figure/table}\dl{you never address the choice of $\mathcal{R}$ is it normal? sounded like a crucial point of Th. 1}\js{i think i mentioned r in thm1; outside i did not mention because of surrogate argument is entirely handwavy (because we cannot prove for outside R)}

==> arXiv Submission/6_discussion.tex <==
\section{Discussion}
We propose a model-free imitation learning algorithm for multi-agent settings that leverages recent advances in adversarial training; the algorithm is agnostic to the competitive/noncompetitive structure of the environment, but allows for incorporating a prior when it is available. Experimental results demonstrate that it is able to imitate complex behaviors in high-dimensional environments with both cooperative and adversarial interactions.
%While the proposed approach allows us to recover the expert policy, there are two main limitations. On the one hand, we are not considering the entire space of $\mb{MAIRL}(\pi_E)$ or even verifying that $\min f_r(\pi_E, V)$ is zero for all proposed reward functions. On the other hand, the problem with MARL being non-injective persists, and training an entirely new policy over the recovered rewards could still lead to policies that do not behave like experts; it might be possible to use an ensemble of reward functions to prevent this.
%%However, under the current assumptions, this seems to be a necessary sacrifice for computational efficiency. 
An interesting research direction is to explore new techniques for gathering expert demonstration; for example, when the expert is allowed to aid the agents by participating in part of the agent's learning process~\citep{hadfield2016cooperative}. 

==> arXiv Submission/cmd.tex <==
\usepackage[utf8]{inputenc}
\usepackage{float}
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{wrapfig}
% \usepackage{subcaption}
\usepackage{placeins}
\usepackage[english]{babel}
\usepackage{url}
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{wrapfig}
\usepackage{bm}
\usepackage{psfrag}
\usepackage{tikz}
\usepackage{epstopdf}
\usepackage{xcolor}
\usepackage{adjustbox}

\newcommand{\beq}[1][\vspace{0.3em}]{#1\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\rbx}[2][!]{
	\resizebox{#1}{!}{$#2$}	
}
\newcommand{\eqs}[1]{\begin{align}#1\end{align}}
\newcommand{\mat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bit}{\vspace{0mm}\begin{itemize}}
\newcommand{\eit}{\vspace{0mm}\end{itemize}}
\newcommand{\ben}{\vspace{0mm}\begin{enumerate}}
\newcommand{\een}{\vspace{0mm}\end{enumerate}}

\newcommand{\Av}[0]{{{\bf A}}}
\newcommand{\Bv}[0]{{{\bf B}}}
\newcommand{\Cv}[0]{{{\bf C}}}
\newcommand{\Dv}[0]{{{\bf D}}}
\newcommand{\Ev}[0]{{{\bf E}}}
\newcommand{\Fv}[0]{{{\bf F}}}
\newcommand{\Gv}[0]{{{\bf G}}}
\newcommand{\Hv}[0]{{{\bf H}}}
\newcommand{\Iv}[0]{{{\bf I}}}
\newcommand{\Jv}[0]{{{\bf J}}}
\newcommand{\Kv}[0]{{{\bf K}}}
\newcommand{\Lv}[0]{{{\bf L}}}
\newcommand{\Mv}[0]{{{\bf M}}}
\newcommand{\Nv}[0]{{{\bf N}}}
\newcommand{\Ov}[0]{{{\bf O}}}
\newcommand{\Pv}[0]{{{\bf P}}}
\newcommand{\Qv}[0]{{{\bf Q}}}
\newcommand{\Rv}[0]{{{\bf R}}}
\newcommand{\Sv}[0]{{{\bf S}}}
\newcommand{\Tv}[0]{{{\bf T}}}
\newcommand{\Uv}[0]{{{\bf U}}}
\newcommand{\Vv}[0]{{{\bf V}}}
\newcommand{\Wv}[0]{{{\bf W}}}
\newcommand{\Xv}[0]{{{\bf X}}}
\newcommand{\Yv}[0]{{{\bf Y}}}
\newcommand{\Zv}[0]{{{\bf Z}}}

\newcommand{\av}[0]{{{\bf a}}}
\newcommand{\bv}[0]{{{\bf b}}}
\newcommand{\cv}[0]{{{\bf c}}}
\newcommand{\dv}[0]{{{\bf d}}}
\newcommand{\ev}[0]{{{\bf e}}}
\newcommand{\fv}[0]{{{\bf f}}}
\newcommand{\gv}[0]{{{\bf g}}}
\newcommand{\hv}[0]{{{\bf h}}}
\newcommand{\iv}[0]{{{\bf i}}}
\newcommand{\jv}[0]{{{\bf j}}}
\newcommand{\kv}[0]{{{\bf k}}}
\newcommand{\lv}[0]{{{\bf l}}}
\newcommand{\mv}[0]{{{\bf m}}}
\newcommand{\nv}[0]{{{\bf n}}}
\newcommand{\ov}[0]{{{\bf o}}}
\newcommand{\pv}[0]{{{\bf p}}}
\newcommand{\qv}[0]{{{\bf q}}}
\newcommand{\rv}[0]{{{\bf r}}}
\newcommand{\sv}[0]{{{\bf s}}}
\newcommand{\tv}[0]{{{\bf t}}}
\newcommand{\uv}[0]{{{\bf u}}}
\newcommand{\vv}[0]{{{\bf v}}}
\newcommand{\wv}[0]{{{\bf w}}}
\newcommand{\xv}[0]{{{\bf x}}}
\newcommand{\yv}[0]{{{\bf y}}}
\newcommand{\zv}[0]{{{\bf z}}}
\newcommand{\epsilonv}[0]{{{\bf \epsilon}}}
\newcommand{\piv}[0]{{\bm{\pi}}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\mb}[1]{\mbox{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}

\providecommand{\abs}[1]{\,\lvert#1\rvert\,}
\providecommand{\norm}[1]{\,\lVert#1\rVert \,}
\newcommand{\Var}{\operatorname{Var}}

\newcommand{\Lim}[1]{\raisebox{0.5ex}{\scalebox{0.8}{$\displaystyle \lim_{#1}\;$}}}

\providecommand{\tightlist}{%
	\setlength{\itemsep}{2pt}\setlength{\parskip}{2pt}}

\providecommand{\js}[1]{{\color{red} [JS: #1]}}
\providecommand{\s}[1]{{\color{blue} [SE: #1]}}
\providecommand{\hr}[1]{{\color{blue} [HR: #1]}}
\providecommand{\se}[1]{{\color{blue} [SE: #1]}}
\providecommand{\dl}[1]{{\color{purple} [DL: #1]}}
\newcommand{\vh}[0]{{{\hat{v}}}}
\newcommand{\qh}[0]{{{\hat{q}}}}
